Recurrent Neural Language Models as Probabilistic Finite-state Automata

Studying language models (LMs) in terms of well-understood formalisms allows us to precisely characterize their abilities and limitations. Previous work has investigated the representational capacity of recurrent neural network (RNN) LMs in terms of their capacity to recognize unweighted formal languages. However, LMs do not describe unweighted formal languages -- rather, they define \emph{probability distributions} over strings. In this work, we study what classes of such probability distributions RNN LMs can represent, which allows us to make more direct statements about their capabilities. We show that simple RNNs are equivalent to a subclass of probabilistic finite-state automata, and can thus model a strict subset of probability distributions expressible by finite-state models. Furthermore, we study the space complexity of representing finite-state LMs with RNNs. We show that, to represent an arbitrary deterministic finite-state LM with $N$ states over an alphabet $\alphabet$, an RNN requires $\Omega\left(N |\Sigma|\right)$ neurons. These results present a first step towards characterizing the classes of distributions RNN LMs can represent and thus help us understand their capabilities and limitations.

==> sections/alphabet-bounds.tex <==
In this section, we provide a family of \dpfsaAcr{}s which require a \hernnAcr{} LM whose size must scale linearly with the size of the alphabet. 
We also provide a sketch of the proof of why a compression in $\nsymbols$ is not possible.
Let $\wfsa_N = \left(\alphabet_N, \set{0, 1}, \set{0}, \set{1}, \trans_N\right)$ be an FSA over the alphabet $\alphabet_N = \set{\sym_1, \ldots, \sym_N}$ such that $\trans_N = \set{\uwedge{0}{\sym_1}{1}} \cup \set{\uwedge{0}{\sym_\idx}{2}\mid \idx = 2, \ldots N}$ (see \cref{fig:log-sigma-counterexample}).
\begin{figure}
    \centering
    % \footnotesize
    \begin{tikzpicture}[node distance = 16mm]
    \node[state, initial] (q0) [] { $0$ }; 
    \node[state] (q1) [right = of q0, yshift=10mm] { $1$ }; 
    \node[state, accepting] (q2) [right = of q0, yshift=-10mm] { $2$ }; 
    \draw[transition] (q0) edge[below, sloped, bend right] node{ $\sym_2,\ldots,\sym_N$ } (q2) 
    (q0) edge[below, sloped, bend left] node{ $\sym_1$ } (q1);
    \end{tikzpicture}
    \caption{The FSA $\wfsa_N$.}
    \label{fig:log-sigma-counterexample}
\end{figure}

Clearly, to be able to correctly represent all local distributions of the \dpfsaAcr{}, the \hernnAcr{} LM must contain a representation of each possible state of the \dpfsaAcr{} in a unique hidden state.
On the other hand, the only way that the \hernnAcr{} can take into account the information about the current state $\qt$ of the simulated FSA $\wfsa$ is through the hidden state $\hiddStatet$.
The hidden state, in turn, only interacts with the recurrence matrix $\recMtx$, which does not have access to the current input symbol $\symtplus$.
The only interaction between the current state and the input symbol is thus through the addition in $\recMtx \hiddStatet + \inMtx \onehot{\symtplus}$. 
This means that, no matter how the information about $\qt$ is encoded in $\hiddStatet$, in order to be able to take into account all possible transitions stemming in $\qt$ (before taking into account $\symtplus$), $\recMtx \hiddStatet$ must activate \emph{all} possible next states, i.e., all children of $\qt$.
On the other hand, since $\inMtx \onehot{\symtplus}$ does not have precise information about $\qt$, it must activate all states which can be entered with an $\symtplus$-transition, just like in Minsky's construction.

In Minsky's construction, the recognition of the correct next state was done by keeping a separate entry (one-dimensional sub-vector) for each possible pair $\qtplus, \symtplus$.
% Since that entry was activated only when this precise pair was active, the 
However, when working with compressed representations of states (e.g., in logarithmic space), a single common sub-vector of size $<\nsymbols$ (e.g., $\log \nsymbols$) has to be used for all possible symbols $\sym \in \alphabet$.
Nonetheless, the interaction between $\recMtx \hiddStatet$ and $\inMtx \onehot{\symtplus}$ must then ensure that only the correct state $\qtplus$ is activated. 
For example, in Minsky's construction, this was done by simply taking the conjunction between the entries corresponding to $\stateq, \sym$ in $\recMtx \hiddStatet$ and the entries corresponding to $\stateq', \sym'$ in $\inMtx \onehot{\sym'}$, which were all represented in individual entries of the vectors.
On the other hand, in the case of the $\log$ encoding, this could intuitively be done by trying to match the $\log \nsymbols$ ones in the representation $\left(\vp\left(\sym\right) \mid \one - \vp\left(\sym\right)\right)$, where $\vp\left(\sym\right)$ represent the binary encoding of $\sym$. 
If the $\log \nsymbols$ ones match (which is checked simply as it would result in a large enough sum in the corresponding entry of the matrix-vector product), the correct transition could be chosen (to perform the conjunction from \cref{fact:and} correctly, the bias would simply be set to $\log\nsymbols - 1$).
However, an issue arises as soon as \emph{multiple} dense representations of symbols in $\inMtx \onehot{\sym}$ have to be activated against the same sub-vector in $\recMtx \hiddStatet$---the only way this can be achieved is if the sub-vector in $\recMtx \hiddStatet$ contains the disjunction of the representations of all the symbols which should be activated with it.
If this sets too many entries in $\recMtx \hiddStatet$ to one, this can result in ``false positives''. 
This is explained in more detail for the \dpfsaAcr{}s in \cref{fig:log-sigma-counterexample} next.

Let $\vr_\idx$ represent any dense encoding of $\sym_\idx$ in the alphabet of $\wfsa_N$ (e.g., in the logarithmic case, that would be $\left(\vp\left(\idx\right) \mid \one - \vp\left(\idx\right)\right)$).
% The nature of the Heaviside activation function limits the
Going from the intuition outlined above, any \hernnAcr{} simulating $\wfsa_N$, the vector $\recMtx \hiddStateZero$ must, among other things, contain a sub-vector corresponding to the states $1$ and $2$.
The sub-vector corresponding to the state $2$ must activate (through the interaction in the Heaviside function) against any $\sym_\idx$ for $\idx = 2, \ldots, N$ in $\wfsa_N$.
This means it has to match all representations $\vr_\idx$ for all $\idx = 2, \ldots, N$.
The only way this can be done is if the pattern for recognizing state $2$ being entered with any $\sym_\idx$ for $\idx = 2, \ldots, N$ is of the form $\vr = \bigvee_{\idx = 2}^N \vr_\idx$.
However, for sufficiently large $N$, $\vr = \bigvee_{\idx = 2}^N \vr_\idx$ will be a vector of all ones---including all entries active in $\vr_1$.
This means that \emph{any} encoding of a symbol will be activated against it---among others, $\sym_1$. 
Upon reading $\sym_1$ in state $1$, the network will therefore not be able to deterministically activate only the sub-vector corresponding to the correct state $1$.
This means that the linear-size encoding of the symbols is, in general, optimal for representing \dpfsaAcr{}s with \hernnAcr{} LMs.\looseness=-1


==> sections/dewdney-indyk.tex <==
Minsky's construction (\cref{sec:minsky}) describes how to represent a \dpfsaAcr{} $\wfsa$ with a \hernnAcr{} of size linear in the number of $\wfsa$'s states.
Importantly, the encoding of the FSA transition function (taken from Minsky's original construction) is decoupled from the parameter defining the probability distribution, $\outMtx$. 
This section describes two asymptotically more space-efficient ways of constructing the component simulating the transition function.
% The two constructions are conceptually similar.
They originate in the work by \citet{Dewdney1977}, who showed that an unweighted FSA $\wfsa = \fsatuple$ can be represented by an \hernnAcr{} of size $\bigO{\nsymbols\nstates^{\frac{3}{4}}}$.
The optimal lower bounds were then more thoroughly studied by \citet{Alon1991EfficientSO}.
Using the same ideas, but a specific trick to compress the size of the processing layer of the RNN further, \citet{Indyk95} later reduced this bound to $\bigO{\nsymbols \sqrt{\nstates}}$, which, as discussed in \cref{sec:space-bounds}, is asymptotically optimal.
Naturally, as shown in \cref{sec:space-bounds}, the space-efficiency gain can not be carried over to the weighted case---that is, the space-efficiency is asymptotically overtaken by the output matrix $\outMtx$.
Nevertheless, for a more complete treatment of the subject, we cover the two compressed constructions of the \hernnAcr{} simulating an unweighted FSA in this section in our notation.
Importantly, given a \dpfsaAcr{}, we focus only on the \emph{underlying FSA}, i.e., the unweighted transition function of the automaton, since by \cref{thm:pfsa-rnn-lower-bound}, the compression can only be achieved with components representing that part of the automaton.
% We also discuss the extension to the weighted case and why it necessarily nullifies the space gains of the more complex construction of the transition function. 

\subsection{Dewdney's Construction} \label{sec:dewdney}
This section describes the construction due to \citet{Dewdney1977} in our notation.
Since some of the parts are very similar to the construction due to \citet{Indyk95}, those parts are reused in \cref{sec:indyk} and introduced more generally.

\paragraph{Representing states of the FSA.}
Let $\wfsa = \fsatuple$ be a deterministic FSA.
Recall that Minsky's construction encodes the $\wfsa$'s current state as a one-hot encoding of the state-symbol pair.
The construction due to \citet{Dewdney1977}, on the other hand, represents the states separately from the symbols.
It encodes the states with \emph{two-hot representations} by using the coefficients of what we call a square-root state representation.
This results in representations of states of size $\bigO{\sqrt{\nstates}}$.
% : instead of representing the state-symbol pairs as one-hot encodings of size $\bigO{\nsymbols \nstates}$ as in \citet{Minsky1954}, individual states are represented as two-hot encodings of size $\bigO{\sqrt{\nstates}}$.
The input symbols are incorporated into the hidden state \emph{separately}.\footnote{This again adds a factor $\nsymbols$ to the size of the hidden state, as we discuss later.}
\begin{definition}
    Let $\wfsa = \fsatuple$ be an FSA and $\srNstates \defeq \ceil{\sqrt{\nstates}}$.
    We define the \defn{square-root state representation} of $\wfsa$'s states $\stateq \in \states$ as\footnote{Notice that $\phitwoFun{\stateq}$ represents the coefficients of the expression of $\stateq \in \N$ in base $\srNstates$.} 
    \begin{equation}
        \phitwoFun{\stateq} \defeq \left(\floor{\frac{\stateq}{\srNstates}}, \stateq\!\mod\!\srNstates\right).
    \end{equation}
    We denote the inverse of $\phitwo$ with $\phitwoInv$ and further define for $k \in \Zmod{\srNstates}$
    \begin{equation}
        \phitwoInvFun{k, \cdot} \defeq \set{\stateq \in \states \mid \evvarphi_0 = k \text{ where } \phiCoor = \phitwoFun{\stateq}}
    \end{equation}
    and $\phitwoInvFun{\cdot, k}$ analogously.
\end{definition}
Specifically, we will denote $\phitwoInvFun{k, \cdot}$ and $\phitwoInvFun{\cdot, k}$ with $k$ in the $j\textsuperscript{th}$ position (with $\idxj \in \Zmod{2}$, $0$ for $\phitwoInvFun{k, \cdot}$ and $1$ for $\phitwoInvFun{\cdot, k}$) as $\compMtx{\idxk}{\idxj}$.

We can think of the function $\phitwo$ as representing states of the FSA in a two-dimensional space $\Zmod{\srNstates} \times \Zmod{\srNstates}$.
However, to efficiently simulate $\wfsa$ with an \hernnAcr{}, it is helpful to think of $\phitwoFun{\stateq}$ in two different ways: as a vector $\vv \in \Nzero^{2 \nstates}$, or as a matrix in $\BQQ$ in the following sense.
\begin{definition} \label{def:vector-matrix-state-representation}
    Given a square-root state representation function $\phitwo$, we define the \defn{vector representation} of the state $\stateq \in \states$ as the vector $\qvectv{\stateq} \in \BtwoQ$ with
    \begin{align}
        \qvectv{\stateq}_{\evvarphi_0} &= 1 \\
        \qvectv{\stateq}_{\srNstates + \evvarphi_1} &= 1,
    \end{align}
    where $\phiCoor = \left(\evvarphi_0, \evvarphi_1\right) = \phitwoFun{\stateq}$, and all other entries $0$.
    Furthermore, we define the \defn{matrix representation} of the state $\stateq \in \states$ as the matrix $\mB \in \BQQ$ with 
    \begin{equation}
        \qMtx{\stateq}_{\evvarphi_0 \evvarphi_1} = 1
    \end{equation} 
    and all other entries $0$.
\end{definition}
Dewdney's construction also heavily relies on the representations of sets of states.
We define those additively.
\begin{definition} \label{def:matrix-state-set-representation}
    Let $\stateSet \subseteq \states$ be a set of states.
    We define the vector representation of $\stateSet$ as the vector
    \begin{equation}
        \qvectv{\stateSet} \defeq \bigvee_{\stateq \in \states} \qvectv{\stateq}.
    \end{equation}
    Similarly, we define the matrix representation of $\stateSet$ as the matrix
    \begin{equation}
        \qMtx{\stateSet} \defeq \bigvee_{\stateq \in \states} \qMtx{\stateq}.
    \end{equation}
\end{definition}

To help understand the above definitions, we give an example of a FSA and the representations of its states.
\begin{example}
Consider the FSA in \cref{fig:dewdney-def-fsa}, for which $\srNstates = \ceil{\sqrt{\nstates}} = \ceil{\sqrt{3}} = 2$, meaning that 
\begin{equation}
    \phitwoFun{0} = \left(0, 0\right)
    \qquad \phitwoFun{1} = \left(0, 1\right)
    \qquad \phitwoFun{2} = \left(1, 0\right),
\end{equation}
resulting in the state-to-vector mapping\footnote{Despite the notation $(\ldots \mid \ldots)$, we assume we are working with column vectors.} 
\begin{align}
    \qvectv{0} &= \begin{pmatrix}
        1 & 0 & \mid & 1 & 0
    \end{pmatrix} \\
    \qvectv{1} &= \begin{pmatrix}
        1 & 0 & \mid & 0 & 1
    \end{pmatrix} \\
    \qvectv{2} &= \begin{pmatrix}
        0 & 1 & \mid & 1 & 0
    \end{pmatrix},
\end{align}
and the state-to-matrix mapping
\begin{equation}
    \qMtx{0} = \begin{pmatrix}
        1 & 0 \\
        0 & 0
    \end{pmatrix}
    \qquad \qMtx{1} = \begin{pmatrix}
        0 & 1 \\
        0 & 0
    \end{pmatrix}
    \qquad \qMtx{2} = \begin{pmatrix}
        0 & 0 \\
        1 & 0 
    \end{pmatrix}.
\end{equation}
The two components of the vector representations separated by ``$\mid$'' denote the two halves of the representation vectors, corresponding to the two components of $\phitwoFun{\stateq}$.

\begin{figure}
    % \scriptsize
    \centering
    \begin{tikzpicture}[node distance = 10mm]
    \node[state] (q0) [] { $0$ }; 
    \node[state] (q1) [right = of q0, yshift=-10mm] { $1$ }; 
    \node[state] (q2) [right = of q0, yshift=10mm] { $2$ }; 
    \draw[transition] (q0) edge[below, sloped, bend right] node{ $\syma$ } (q1) 
    (q0) edge[above, sloped, bend left] node{ $\symb$ } (q2)
    (q1) edge[right, bend right] node{ $\syma$ } (q2) 
    (q2) edge[above, sloped, bend left] node{ $\symb$ } (q0) 
    (q1) edge[right, loop right] node{ $\symb$ } (q1) ;
    \end{tikzpicture}
    \caption{An example of a fragment of an FSA.}
    \label{fig:dewdney-def-fsa}
\end{figure}
    
\end{example}

\paragraph{High-level idea of Dewdney's construction.}
Given these definitions, the intuition behind Dewdney's construction of an \hernnAcr{} simulating an FSA $\wfsa$ is the following:
\begin{enumerate}
    \item Represent $\wfsa$'s states as vectors in $\Btwos$, or, equivalently, matrices in $\Bss$.
    \item For each $\stateq \in \states$, construct the matrix representation of the set of $\sym$-parents $\qMtx{\qPreds{\stateq, \sym}}$ for all $\sym \in \alphabet$.
    \item To simulate $\wfsa$'s transition function $\trans$, compare the representation of the current state $\qt$ with all constructed parent matrices $\qMtx{\qPreds{\stateq, \symt}}$ given the current input symbol $\symt$.
    Activate the two-hot representation of the (unique) state $\qtplus$ for which the representation of $\qt$ was detected in $\qtplus$'s parent matrix for symbol $\symt$, $\qMtx{\qPreds{\qtplus, \symt}}$.
    % Since $\qt$ will be in the set of the parents of the correct next state $\qtplus$, and will thus be included in $\qtplus$'s parent matrix, .
    % Therefore, set the next hidden state to the representation of the state whose parent matrix given $\symt$ included $\qt$.
\end{enumerate}

\paragraph{Simulating the transition function of an FSA by detecting preceding states.}
We elaborate on the last point above since it is the central part of the construction.\footnote{Later, we will see that \citet{Indyk95} uses the exact same idea for simulating $\trans$.}
The idea of simulating the transition function $\trans$ is reduced to detecting \emph{whose parent} given the current input symbol $\symt$ is currently active---naturally, this should be the state active at $\tstep + 1$. 
Concretely, consider again the FSA $\wfsa$ in \cref{fig:dewdney-def-fsa}.
The parents of the three states, indexed by the incoming symbols are: for $0$ $\left\{\symb: 2\right\}$, for $1$ $\left\{\syma: 1, \symb: 0\right\}$, and for $2$ $\left\{\syma: 1, \symb: 0\right\}$.
Suppose that at some time $\tstep$, $\wfsa$ is in state $0$ and is reading in the symbol $\symb$.
Then, since the state $0$ is the $\symb$-parent of the state $2$, we know that at time $\tstep + 1$, $\wfsa$ will be in state $2$.
This principle can be applied more generally: To determine the state of an FSA at time $\tstep + 1$, we simply have to somehow detect whose \emph{parent} is active at time $\tstep$ \emph{given the current input symbol} at time $\tstep$.

The crux of Dewdney's construction is then the following:\footnote{Again, the same applies to \citet{Indyk95}.} How do we, using only the Elman update rule, determine whose $\symt$-parent is active at time $\tstep$?
% That will be the new state of the FSA and therefore dictate the new state of the \hernnAcr{}.
This can be done by \emph{detecting} which parent matrix $\qMtx{\qPreds{\stateq, \symt}}$ the representation of the current state $\qt$ is included in in the sense that if $\phitwoFun{\qt} = \phiCoor$, it holds that $\qMtx{\qPreds{\stateq, \symt}}_{\evvarphi_0\evvarphi_1} = 1$.
To be able to formally talk about the detection of a representation in a set of parents, we define several notions of \defn{matrix detection}.

Informally, we say that a matrix is easily detectable if the presence of its non-zero elements can be detected using a single neuron in the hidden layer of a \hernnAcr{}.
\begin{definition}
Let $\mB \in \BDD$ be a binary matrix.
We say that $\mB$ is \defn{easily detectable} if there exist $\vw \in \Q^{2 D}$ and $b \in \Q$ (neuron coefficients) such that 
\begin{equation}
    \sigmoidFun{\innerProd{\ve_{ij}}{\vw} + b} = 1 \iff \emB_{ij} = 1,
\end{equation}
where $\ve_{ij} = \begin{pmatrix} \ve_i & \mid & \ve_j \end{pmatrix}$ refers to the $2 D$-dimensional vector with $1$'s at positions $i$ and $D + j$.
In words, this means that the neuron defined by $\vw, b$ fires on the input $\ve_{ij}$ if and only if $\emB_{ij} = 1$.
% Equivalently, this means that the neuron defined by $\vw$ and $b$ fires if and only if the vector $\begin{pmatrix} \ve_i & \mid & \ve_j \end{pmatrix}$ encodes a position with a $1$ in the matrix $\mB$.
\end{definition}
We define detectable matrices as the matrices which can be detected using a conjunction of two neurons.
\begin{definition}
Let $\mB \in \BDD$ be a binary matrix.
We say that $\mB$ is \defn{detectable} if there exist $\vw_1, \vw_2 \in \Q^{2 D}$ and $b_1, b_2 \in \Q$ such that 
\begin{equation}
    \sigmoidFun{\innerProd{\ve_{ij}}{\vw_1} + b_1} = 1 \wedge \sigmoidFun{\innerProd{\ve_{ij}}{\vw_2} + b_2} = 1 \iff \emB_{ij} = 1.
\end{equation}
\end{definition}
Furthermore, we say that a matrix is (easily) \defn{permutation-detectable} if there exist permutation matrices $\mP$ and $\mQ$ such that $\mP \mB \mQ$ is (easily) detectable.

Intuitively, this means that one can effectively replace an easily detectable matrix $\mB$ with \emph{a single neuron}: Instead of specifying the matrix explicitly, one can simply detect if an entry $\emB_{ij}$ of $\mB$ is $1$ by passing $\ve_{ij}$ through the neuron and seeing if it fires. 
This reduces the space complexity from $D^2$ to $2D$.
Similarly, one can replace a detectable matrix with \emph{two} neurons.
As shown in \cref{fact:and}, the required conjunction of the two resulting neurons can then easily be performed by a third (small) neuron, meaning that a detectable matrix is effectively represented by a two-layer MLP.
% Intuitively, this means that the non-zero elements of the matrix can be detected\anej{rethink} by the conjunction of two neurons (which can be altogether performed by a two-layer MLP).

An example of easily detectable matrices are the so-called \defn{northwestern} matrices.
% Dewdney's construction makes heavy use of them.
\begin{definition}
    A matrix $\mB \in \BDD$ is \defn{northwestern} if there exists a vector $\balpha$ with $|\balpha| = D$ and $D \geq \alpha_1 \geq \ldots \geq \alpha_D \geq 0$ such that 
    \begin{equation}
        \emB_{ij} = 1 \iff j \leq \alpha_i.
    \end{equation}
\end{definition}
Intuitively, northwestern matrices contain all their ones contiguously in their upper left (northwest) corner.
An example of a northwestern matrix for $\balpha = \begin{pmatrix}
    2 & 1 & 1
\end{pmatrix}$ is 
\begin{equation}
    \mB = \begin{pmatrix}
        1 & 1 & 0 \\ 1 & 0 & 0 \\ 1 & 0 & 0
    \end{pmatrix}.
\end{equation}

\begin{lemma} \label{lem:nw-matrices-easily-detectable}
    Northwestern matrices are easily detectable.
\end{lemma}
\begin{proof}
    Define 
    \begin{equation*}
        \vw \defeq \begin{pmatrix}
            \balpha & \mid & D & \ldots & 1
        \end{pmatrix}
    \end{equation*}
    and $b = -D$.
    It is easy to see that for any $\ve_{ij}$ where $\mB_{ij} = 1$, it holds that
    \begin{align*}
        & \innerProd{\ve_{ij}}{\vw} = \alpha_i + (D - j + 1) \geq j + D - j + 1 = D + 1 \\
        & \implies \heavisideFun{\innerProd{\ve_{ij}}{\vw} + b} = \heavisideFun{\innerProd{\ve_{ij}}{\vw} - D} = 1.
    \end{align*}
    
    On the other hand, for $\emB_{ij} = 0$, we have
    \begin{align*}
        & \innerProd{\ve_{ij}}{\vw} = \alpha_i + (D - j + 1) < j + D - j + 1 = D \\
        & \implies \heavisideFun{\innerProd{\ve_{ij}}{\vw} + b} = \heavisideFun{\innerProd{\ve_{ij}}{\vw} - D} = 0.
    \end{align*}
\end{proof}

A more general useful class of detectable matrices are line matrices \citep{Dewdney1977}.
\begin{definition} \label{def:line-matrix}
    A binary matrix $\mB \in \BDD$ is a \defn{line matrix} if any of the following conditions hold:
    \begin{enumerate}
        \item All $\mB$'s ones lie either in the same row ($\mB$ is a \defn{row matrix}) or in the same column ($\mB$ is a \defn{column matrix}).
        % \item All $\mB$'s ones lie in the same column ($\mB$ is a \defn{column matrix}).
        \item $\mB$ is a \emph{transversal}, i.e., a matrix in which there is at most one $1$ in any column and row.
    \end{enumerate}
\end{definition}

\begin{lemma} \label{lem:lines-detectable}
    Row and column matrices are easily permutation-detectable.
\end{lemma}
\begin{proof}
    Let $i, N \in \Zmod{D}$ and $\mB$ be a row matrix with $\mB_{ij_n} = 1$ for $n \in \Zmod{N}$, i.e., a row matrix with all its ones in the $i^\text{th}$ row.
    Define $\mP \in \BDD$ as $\emP_{1 i} = 1$ and $0$ elsewhere and $\mQ \in \BDD$ with $\mQ_{j_n n} = 1$ and $0$ elsewhere.
    Then, $\mP \mB \mQ$ contains all its $1$ in its northwestern corner (contiguously in the first row) and is thus easily detectable.
    Let $\vw \defeq \begin{pmatrix} \balpha & \mid & D & \ldots & 1 \end{pmatrix}$, $b = D$ be the neuron weights from \cref{lem:nw-matrices-easily-detectable}.
    Define $\vw' \defeq \begin{pmatrix} \mP^\top \balpha & \mid & \mQ(D & \ldots & 1) \end{pmatrix}$, $b' = D$.
    It is easy to see that this ``rearranges'' the components of the neuron recognizing the northwestern matrix $\mP \mB \mQ$ to make them recognize the original matrix, meaning that the neuron defined by $\vw'$ and $b'$ recognizes the line matrix.
    The proof for a column matrix is analogous.
\end{proof}

\begin{lemma} \label{lem:trans-detectable}
    Transversals are permutation-detectable.
\end{lemma}
\begin{proof}
    The core idea of this proof is that every transversal can be permuted into a diagonal matrix, which can be written as a Hadamard product of a lower-triangular and an upper-triangular matrix.

    Let $\mB$ be a transversal.
    Pre-multiplying $\mB$ with its transpose $\mP \defeq \mB^\top$ results in a diagonal matrix.
    It is easy to see that $\mP \mB$ can be written as a Hadamard product $\mH_1 \otimes \mH_2$ of a lower-triangular matrix $\mH_1$ and an upper-triangular matrix $\mH_2$.
    Both are easily permutation detectable.
    A conjunction of the neurons detecting $\mH_1$ and $\mH_2$ (again, performed by another neuron) detects the original matrix $\mB$.
    In the following, we will refer to $\mH_1$ and $\mH_2$ as the \emph{factors} of the transversal.
\end{proof}

Crucially, any binary matrix $\mB \in \BDD$ can be decomposed into a set of line matrices $\sB$ whose disjunction is $\mB$: $\bigvee_{\mM \in \sB} \mM = \mB$.
It is easy to see that $\mB_{ij} = 1$ if and only if there exists $\mM \in \sB$ such that $\mM_{ij} = 1$.
This means that non-zero entries of \emph{any} $\mB \in \BDD$ decomposed into the set of line matrices $\sB$ can be detected using an MLP in two steps: 
\begin{enumerate}
    \item Detect the non-zero entries of the individual line matrices from the decomposition $\sB$ (which are, as shown above, detectable).
    \item Take a disjunction of the detections of the individual line matrices to result in the activation of the original matrix.
\end{enumerate}
The disjunction can again be performed by applying another 2-layer MLP to the activations of the line matrices.
An important consideration in both Dewdney's as well as Indyk's construction later will be \emph{how large} $\sB$ has to be.

% With these definitions and results, we are now able to formally describe Dewdney's construction and its generalization to the weighted case.
% We can now finally formally describe Dewdney's construction.
\paragraph{Using matrix decomposition and detection for simulating the transition function.}
We now describe how Dewdney's construction uses matrix detection based on the decomposition of matrices into line matrices to simulate an FSA using an \hernnAcr{}.
From a high level, the update steps of the \hernnAcr{} will, just like in Minsky's construction, simulate the transition function of the simulated FSA.
However, in contrast to the Minsky construction, in which each transition step in the FSA was implemented by a \emph{single} application of the Elman update rule, here, a single transition in the FSA will be implemented using \emph{multiple} applications of the Elman update rule, the end result of which is the activation of the two-hot representation of the appropriate next state.
Nonetheless, there are, abstractly, two sub-steps of the update step, analogous to the Minsky construction (cf. \cref{fig:minsky-overview}):
\begin{enumerate}
    % \item Detect activations of the line matrices.
    % \item Combine the activations of the line matrices into the activations of all possible next states.
    \item Detect the activations of all possible next states, considering any possible input symbol (performed by the term $\recMtx \hiddStatet$ in Minsky's construction).
    \item Filter the activations of the next states by choosing only the one transitioned into by a $\symt$-transition (performed by conjoining with the term $\inMtx \onehot{\symt}$ in Minsky's construction).
\end{enumerate}
The novelty of Dewdney's construction comes in the first sub-step: How can the Elman update step be used to activate the two-hot representation of $\qt$'s children?
% How do we activate all possible next states from the current state $\qt$ ($\qt$'s children)?
As alluded to, this relies on the pre-computed parent matrices $\qPreds{\stateq, \sym}$ (cf. \cref{def:vector-matrix-state-representation}).
% of all possible states and for all possible symbols, $\qPreds{\stateq, \sym}$.
% Instead of activating the individual one-hot encodings of the state-symbol pairs of the children (as done in Minsky's construction), the hidden state update rule activates the \emph{two-hot representation} of the next state of the simulated FSA.
% This reduces the size of the hidden state from $\bigO{\nsymbols \nstates}$ to $\bigO{\nsymbols \sqrt{\nstates}}$.\footnote{Additional units are required for ``processing'', as we describe later.}
% These are then \emph{combined} and compressed in a specific way: instead of detecting the parent matrices of individual state-symbol pairs, the activations of the hidden state in Dewdney's construction detect the activations of the dimensions of the \emph{vector representation} (cf. \cref{def:vector-matrix-state-representation}) of the next state.
% More concretely, exactly the two components corresponding to the two-hot representation of the next state are activated.
The parent matrices of individual states are compressed (disjoined) into component-activating matrices, the representation matrices of the parents of specific \emph{sets} of states (cf. \cref{def:matrix-state-set-representation}), defined through the function $\phitwo$ in the following sense.
% This allows us to define the component-activating matrices as follows.
\begin{definition}
    A \defn{component-activating matrix} is the representation matrix $\mB_{\idxj, \sym, \idxk} \defeq \qMtx{\qPreds{\compMtx{\idxk}{\idxj}, \sym}}$ for some $\idxk \in \Zmod{\frNstates}$ and $\idxj \in \Zmod{2}$.
\end{definition}
% These matrices of interest are \defn{component-activating matrices}, representing the sets $\qPreds{\sQ, \sym}$ for $\sym \in \alphabet$, where either $\sQ = \phitwoInvFun{k, \cdot}$ or $\sQ = \phitwoInvFun{\cdot, k}$ for some $k \in \NTo{\srNstates}$.
% We call such matrices \defn{component-activating matrices}, since, as will become clear shortly, they define one of the two sub-vectors of the \hernnAcr{} hidden state.
Intuitively, the component-activating matrix $\mB_{\idxj, \sym, \idxk}$ is the result of the disjunction of the matrix representations of all $\sym$-parents $\stateq$ of all states $\stateq'$ whose $\idxj\textsuperscript{th}$ component of the vector $\phitwoFun{\stateq'}$ equals $\idxk$.
This results in $2 \nsymbols \srNstates$ matrices.
% , where each matrix, intuitively, detects the activation of a parent of a state with a non-zero entry at a specific entry in the two-hot vector representation of the state ($\idxj$ and $\idxk$), upon reading a specific symbol ($\sym$).
They can be pre-computed and naturally depend on the transition function $\trans$.
The name component-activating matrix is inspired by the fact that each of the matrices ``controls'' the activation of one of the $2 \nsymbols \srNstates$ neurons in a specific sub-vector of the \hernnAcr{} hidden state.
That is, each component-activating matrix controls a particular dimension, indexed by the tuple $\left(\idxj, \sym, \idxk\right)$ for $\idxj \in \B, \sym \in \alphabet, \idxk \in \Zmod{\srNstates}$, in the \defn{data sub-vector} of the \hernnAcr{} hidden state.
As we will see shortly, they contain all the information required for simulating $\wfsa$ with a \hernnAcr{}.
% We will denote the matrix representing the set $\qPreds{\sQ; \sym}$ as $\mB_{x, \sym, k}$, where $x=0$ corresponds to $\sQ = \phitwoInvFun{\cdot, k}$ and $x=1$ to $\sQ = \phitwoInvFun{k, \cdot}$.

To define the transition function of the \hernnAcr{} simulating $\wfsa$, all $2 \nsymbols \srNstates$ component-activating matrices are decomposed into permutation-detectable line matrices (cf. \cref{def:line-matrix}) whose activations are combined (disjoined) into the activations of individual component-activating matrices.
Analogously to above, we will denote the sets of line matrices decomposing the component-activating matrices as $\sB_{\idxj, \sym, \idxk}$, i.e., $\mB_{\idxj, \sym, \idxk} = \bigvee_{\mM \in \sB_{\idxj, \sym, \idxk}} \mM$.
The dimensions of the hidden state corresponding to the activations of the line matrices before they are combined into the activations of the component-activating matrices form the \defn{processing sub-vector} of the \hernnAcr{} hidden state since they are required in the pre-processing steps of the update step to determine the activation of the actual hidden state.
This is schematically drawn in \cref{fig:dewdney-high-level}.
% More concretely, after constructing $\nstates \nsymbols$ parent matrices $\qMtx{\qPreds{\stateq, \sym}}$, we construct $\nstates \nsymbols$ \emph{sets} of line matrices $\qBs{\qPreds{\stateq, \sym}}$, such that for any $\stateq \in \states$ and $\sym \in \alphabet$, it holds that $\sum_{\mM \in \qBs{\qPreds{\stateq, \sym}}} \mM = \qMtx{\qPreds{\stateq, \sym}}$.
% The recurrence and the input matrices of the \hernnAcr{} then ensure that the data and processing components of the hidden state interact correctly to update the hidden state according to the transition function of the FSA.

\begin{figure*}
    \centering
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{figures/Dewdney.pdf}
        \caption{High-level overview of Dewdney's construction. 
        The highlighted \textcolor{ETHBronze}{orange} neuron in the representation of the state from the data sub-vector corresponds to the activation of one of the components of the \textcolor{ETHRed}{red} states (which have in common that their $0\textsuperscript{th}$ component of $\phitwoFun{\stateq}$ is the same). 
        The matrix corresponding to the disjunction of the representations of their \emph{$\sym$-parents} (\textcolor{ETHBlue}{blue} states) is decomposed into two line matrices---a transversal and a column matrix. 
        The non-zero elements of the former can be detected by a conjunction of two neurons while the non-zero elements of the latter can be detected directly by a single neuron. 
        Those activations are then disjoined to result in the activation in the \textcolor{ETHBronze}{orange} neuron.
        The \textcolor{ETHPurple}{purple} neurons in the processing sub-vector are composed of the neurons in the networks implementing the detection of line matrices and their conjunctions and disjunctions (also shown in \textcolor{ETHPurple}{purple}).}
        \label{fig:dewdney-high-level}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \centering
        \begin{tikzpicture}
          \matrix[matrix of math nodes, column sep=0.6cm, row sep=5mm, nodes={minimum width=1.5cm}] (mat) {
            \begin{tikzpicture}[node distance = 6mm]
            \footnotesize
            \node[state, fill=ETHPurple!30, draw=ETHPurple!80] (q){ $\stateq$ }; 
            \node[state] (q1) [above right = of q] { $\stateq'$ }; 
            \node[state] (q2) [below right = of q] { $\stateq''$ }; 
            \draw[transition] (q) edge[above, sloped] node{ $\syma$ } (q1) 
            (q) edge[above, sloped] node{ $\symb$ } (q2);
            \end{tikzpicture}
            &
            &
            \begin{tikzpicture}[node distance = 6mm]
            \footnotesize
            \node[state] (q){ $\stateq$ }; 
            \node[state, fill=ETHPetrol!20] (q1) [above right = of q] { $\stateq'$ }; 
            \node[state, fill=ETHPetrol!20] (q2) [below right = of q] { $\stateq''$ }; 
            \draw[transition] (q) edge[ETHPetrol, above, sloped] node{ $\syma$ } (q1) 
            (q) edge[ETHPetrol, above, sloped] node{ $\symb$ } (q2);
            \end{tikzpicture} &
            \begin{tikzpicture}[node distance = 6mm]
            \footnotesize
            \node[state] (q){ $\stateq$ }; 
            \node[state, fill=ETHGreen!30, draw=ETHGreen!80] (q1) [above right = of q] { $\stateq'$ }; 
            \node[state] (q2) [below right = of q] { $\stateq''$ }; 
            \draw[transition] (q) edge[ETHGreen, above, sloped] node{ $\syma$ } (q1) 
            (q) edge[above, sloped] node{ $\symb$ } (q2);
            \end{tikzpicture} \\
            \begin{pmatrix}
              \textcolor{ETHRed}{\qvectv{\stateq}} \\ \vp
            \end{pmatrix} &
            \begin{pmatrix}
              \qvectv{\stateq} \\ \textcolor{ETHRed}{\vp'}
            \end{pmatrix} &
            \begin{pmatrix}
              \textcolor{ETHRed}{\qvectv{\set{\stateq', \stateq''}}} \\ \vp''
            \end{pmatrix} &
            \begin{pmatrix}
              \textcolor{ETHRed}{\qvectv{\stateq'}} \\ \vp'''
            \end{pmatrix} \\
          };
          
          \foreach \i in {1,...,4} {
            \node at ([yshift=0.25cm]mat-2-\i.north) {\small Phase \i};
          }
          
          \foreach \i in {1,...,3} {
            \draw [->,thick] (mat-2-\i.east) -- (mat-2-\the\numexpr\i+1\relax.west);
          }
        \end{tikzpicture}
        \caption{A high-level illustration of how the transition function of the FSA is implemented in Dewdney's construction on an example of an FSA fragment, where the simulated automaton is initially in the state $\stateq$ and reads the symbol $\syma$, transitioning to $\stateq'$.
        The components whose changes are relevant at a given step are \textcolor{ETHRed}{highlighted}.
        Starting in the state $\stateq$, which is stored in the data sub-vector $\qvectv{\stateq}$, in the first sub-step, the processing bits of the appropriate line matrices are activated ($\vp'$).
        Next, the activated line matrices are used to activate the representations of all of $\stateq$'s children in the data sub-vector ($\qvectv{\set{\stateq', \stateq''}}$). 
        Lastly, these representations are conjoined with the states reachable by the symbol $\syma$, resulting in the representation of the state $\stateq$ in the data sub-vector ($\qvectv{\stateq}$).
        }
        \label{fig:dewdney-phases}
    \end{subfigure}
\end{figure*}



For any component-activating matrix $\mB$ decomposed into the set of line matrices $\sB$, we know by \cref{lem:lines-detectable,lem:trans-detectable} that all $\mM \in \sB$ are detectable by a single-layer MLP.
By adding an additional layer to the MLP, we can disjoin the detections of $\mM \in \sB$ into the detection of $\mB$.
More abstractly, this MLP, therefore, detects the activation of \emph{one} of the $2 \nstates \srNstates$ cells of the data sub-vector of the \hernnAcr{} hidden state---all of them together then form the two-hot encoding of all possible next states of the FSA (before taking into account the input symbol).
Designing $2 \nstates \srNstates$ such single-values MLPs, therefore, results in an MLP activating the two-hot representations of all possible next states of the simulated FSA.
% Since we can do this for any of the $2 \nstates \srNstates$ component-activating matrices individually, we can build an MLP detecting the activations of all the matrices \emph{individually}.
Conjoining these activations with the input symbol, analogously to how this is done in the Minsky construction, results in the activation of the two-hot representation of only the actual next state of the simulated FSA.
This is illustrated in \cref{fig:dewdney-phases}.

\paragraph{High-level overview of simulating a transition.}
In summary, after decomposing all the component-activating matrices into the sets $\sB_{\idxj, \sym, \idxk}$, the detection of all candidate next states (before considering the input symbol) in the update step of \hernnAcr{} is composed of the following sub-steps.
\begin{enumerate}
    \item Compute the activations of the two \emph{factors} of all the transversals in $\sB_{\idxj, \sym, \idxk}$ for all $\idxj, \sym, \idxk$ (\cref{lem:trans-detectable}).
    \item Conjoin the activations of the two factors into the activations of the transversals (\cref{lem:trans-detectable}).
    \item Compute the activations of the column and row matrices in $\sB_{\idxj, \sym, \idxk}$ for all $\idxj, \sym, \idxk$  (\cref{lem:lines-detectable}).
    \item Disjoin of the activations of all the line matrices (transversals, row, and column matrices) in $\sB_{\idxj, \sym, \idxk}$ for all $x, \sym, \idxk$ to compute the activations of all $2 \nsymbols \srNstates$ component-activatimg matrices.
\end{enumerate}
This results in the activation of the two-hot representations of all possible next states (i.e., all children of $\qt$).
In the last sub-step of the \hernnAcr{} update step, these are conjoined with the representation of the current input symbol.
This step is very similar to the analogous stage in Minsky's construction, with the difference that here, the non-zero entries of the vector $\inMtx \hiddStatet$ must cover the two-hot representations of the states with an incoming $\symt$-transition.
This conjunction then ensures that among all the children of $\qt$, only the one reached by taking the $\symt$-transition will be encoded in $\hiddStatetplus$.
The construction just described can be summarized by the following lemma.
\begin{lemma} \label{lemma:dewdney-correctness}
    Let $\wfsa = \fsatuple$ be a deterministic FSA.
    Then, Dewdney's construction results in a \hernnAcr{} correctly simulating $\wfsa$'s transition function, i.e, $\hToQFun{\hiddStatet} = \qt$ for all $\tstep$.
\end{lemma}
\begin{proof}
The proof follows the reasoning on the activation of appropriate matrices according to the transition function of the FSA outlined above.
To formally prove the lemma, we would have to follow a similar set of steps to how the correctness of Minsky's construction (\cref{lem:minsky-transitions}) was proved. 
We omit this for conciseness.
\end{proof}

This shows that Dewdeny's construction correctly encodes the FSA in a \hernnAcr{}.
However, its space efficiency remains to be determined. 
As mentioned above, working with two-hot representations of the states means that the data sub-vector is of size $\bigO{\nsymbols \sqrt{\nstates}}$.
However, the construction also requires a number of processing dimensions in the processing sub-vector.
To understand the full complexity of the construction, we have to determine the maximal number of processing bits in the \hernnAcr{}.
% The only thing that remains to be investigated is the space-efficiency of the construction.
The first step to the answer is contained in the following lemma, which describes the number of line matrices required to cover an arbitrary binary matrix.
It lies in the core of the efficiency of Dewdney's construction.
% The core of the efficiency of Dewdney's construction lies in the following lemma.
\begin{lemma} \label{lem:line-decomp-lower-bound}
    Let $\mB \in \BDD$ with $N^2$ elements equalling $1$.
    Then, there exists a decomposition $\sB$ of $\mB$ into at most $2 N$ line matrices such that $\bigvee_{\mM \in \sB} \mM = \mB$.
\end{lemma}
\begin{proof}
    Based on \citet{Dewdney1977}.\footnote{The proof in \citet{Dewdney1977} contains a mistake that affects the constant, but not the big-O complexity of the space complexity. It is fixed in this proof.}
    Define the sequence of transversals $\mT_1, \mT_2, \ldots$ where $\mT_\idxi$ is the transversal containing the maximum number of ones in the matrix $\mB_\idxi \defeq \mB - \bigvee_{\idxj = 1}^{\idxi - 1} \mB_{\idxj}$. 
    The transversal containing the maximal number of ones can be found using the maximum matching algorithm.
    Continue this sequence until there are no more ones in $\mB_\idxi$.
    The number of ones in the matrices $\mB_\idxi$, $\norm{\mB_\idxi}_1$, forms a (weakly) decreasing sequence.

    If there are at most $2 N$ transversals in the sequence, the lemma holds.
    Otherwise, we compare the functions $\func\left(\idxi\right) \defeq \norm{\mT_\idxi}_1$ and $\funcg\left(\idxi\right) \defeq 2N - \idxi$.
    \begin{itemize}
        \item If $\func\left(\idxi\right) > \funcg\left(\idxi\right)$ for all $\idxi = 1, \ldots, N$, then $\sum_{\idxi = 1}^{N}\func\left(\idxi\right) = \sum_{\idxi = 1}^{N}\norm{\mT_\idxi}_1 > \sum_{\idxi = 1}^{N} 2N - \idxi = 2N^2 - \frac{1}{2} N (N + 1) \geq N^2$.
        However, the transversals in the decomponsition cannot contain more ones than the original matrix.
        \item We conclude that for some $\idxi \leq N$, $\func\left(\idxi\right) \leq \funcg\left(\idxi\right)$.
        Let $\idxi_0$ be the first such index in $1, \ldots, N$ and $\sL_1 \defeq \set{\mT_1, \ldots, \mT_k}$.
        Since the maximum number of independent ones (in the sense that at most one appears in a single row/column) in $\mB_{\idxi_0 - 1}$ is $\norm{\mT_{\idxi_0}}_1 \leq 2N - \idxi_0$ (those are chosen by the maximum transversal $\mT_{\idxi_0}$).
        By K\"onig's theorem \citep{szárnyas2020graphs}, there is a set of at most $2N - \idxi_0$ column or row matrices $\sL_2 \defeq \set{\mL_{1}, \ldots \mL_{\idxk}}$ with $k \leq 2N - \idxi_0$ which cover $\mB_{\idxi_0 - 1}$.\footnote{Intuitively, since all ones are contained within $\leq 2N - \idxi_0$ rows or columns, they can be simply covered by matrices containing those.} 
        Therefore, $\sL \defeq \sL_1 \cup \sL_2$ constitutes a valid cover of $\mB$ with $\leq N + 2N - \idxi_0 = \bigO{N}$ matrices. 
    \end{itemize}
\end{proof}
We will denote the number of matrices in the line decomposition of a matrix $\mB$ constructed by the greedy procedure from \cref{lem:line-decomp-lower-bound} as $\nLines{\mB}$.
Connecting this lemma to Dewdney's construction, this shows that the number of neurons required to detect the activation of a \emph{single set} $\qPreds{k, \sym}$ grows asymptotically as the square root of the number of ones in the representation matrix $\qMtx{\qPreds{k, \sym}}$---this is how many line matrices the matrix will decompose into.
The size of each neuron is $2 \nsymbols \srNstates$.

This allows us to show how many neurons the entire \hernnAcr{} simulating $\wfsa$ has. 
Since we know that the data sub-vector will always have exactly $2 \nsymbols \srNstates$ cells, we characterize the number of processing cells in the following lemma.
\begin{lemma} \label{lemma:dewdney-bound}
    Let $\wfsa = \fsatuple$ be a deterministic FSA. 
    Then, Dewdney's construction results in a \hernnAcr{} with a hidden state of size $\bigO{\nsymbols \nstates^{\frac{3}{4}}}$.
\end{lemma}
\begin{proof}
    The number of cells in the entire processing sub-vector is simply the sum of the processing neurons of all the data components.
    In the worst case, a single component-activating matrix $\mB$ requires $2 \nLines{\mB} + 1$ neurons ($2$ for each transversal in the decomposition of $\mB$ and an additional one for their disjunction).
    Therefore, enumerating the set of matrices $\set{\mB_{\idxj, \sym, \idxk} \mid \idxj \in \Zmod{2}, \sym \in \alphabet, \idxk \in \Zmod{\srNstates}}$ with $\mB_\idxn$ for $\idxn = 1, \ldots, 2 \nsymbols \srNstates$, the number of neurons required by all component-activating matrices is bounded as follows.
    \begin{equation}
        \sum_{\idxn = 1}^{2 \nsymbols \srNstates} 2 \nLines{\mB_\idxn} + 1 \leq 
        \sum_{\idxn = 1}^{2 \nsymbols \srNstates} 2 \left(2 \ceil{\sqrt{\norm{\mB_\idxn}_1}}\right) + 1 \defeq 
        \sum_{\idxn = 1}^{2 \nsymbols \srNstates} 4 m_\idxn + 1  \label{eq:n-components}
    \end{equation}
    Since the matrices $\mB_\idxn$ contain one non-zero entry for each state-symbol pair, it holds that
    \begin{equation} \label{eq:n-components-constraint}
        \sum_{\idxn = 1}^{2 \nsymbols \srNstates} \norm{\mB_\idxn}_1 \leq \sum_{\idxn = 1}^{2 \nsymbols \srNstates} m^2_\idxn = \nsymbols \nstates
    \end{equation}
    Pretending that $m_\idxn$ can take real values, the value of \cref{eq:n-components} is maximized under the constraint from \cref{eq:n-components-constraint} when all $m_\idxn$ are equal with $m_\idxn = \sqrt{2 \srNstates}$.
    This means that 
    \begin{equation}
        \sum_{\idxn = 1}^{2 \nsymbols \srNstates} 4 m_\idxn + 1 \leq \sum_{\idxn = 1}^{2 \nsymbols \srNstates} 4 \sqrt{2 \srNstates} + 1
        = 8 \nsymbols \srNstates \sqrt{2 \srNstates} + 1
        = \bigO{\nsymbols \nstates^{\frac{3}{4}}},
    \end{equation}
    finishing the proof.
\end{proof}

All results stated in this section can be summarized in the following theorem.
\begin{theorem}
    Let $\wfsa = \fsatuple$ be a deterministic FSA.
    Then, there exists a \hernnAcr{} of size $\bigO{\nsymbols \nstates^{\frac{3}{4}}}$ correctly simulating $\wfsa$.
\end{theorem}
\begin{proof}
    The existence of the RNN follows from the discussion on detectable matrices and \cref{lemma:dewdney-correctness} while the space bound is guaranteed by \cref{lemma:dewdney-bound}.
\end{proof}

\subsection{Indyk's Construction} \label{sec:indyk}
\cref{sec:dewdney} describes a construction of an \hernnAcr{} of size $\bigO{\nsymbols \nstates^\frac{3}{4}}$ simulating an FSA.
While this improves the space efficiency compared to Minsky's construction, it is not asymptotically optimal.
\citet{Indyk95} proved that a \hernnAcr{} simulating an FSA $\wfsa = \fsatuple$ over a binary alphabet $\alphabet = \B$ requires at least $\Omega\left(\sqrt{\nstates}\right)$ hidden dimensions. 
He also provided a construction that achieves this lower bound.
This construction is conceptually very similar to Dewdney's in that it works by activating neurons corresponding to some form of compressed parent matrices (component-activating matrices) and then selecting the transition which matches the input symbol.
Again, it additively covers these matrices with components that are easy to detect, similar to how Dewdney's construction uses line matrices.
However, Indyk's construction defines component-activating matrices based on different sets of states and covers them with a different decomposition---these are the two crucial differences allowing the construction to achieve the optimal lower bound.
% However, the methods of defining component-activating matrices and covering them differ---this is the crucial difference allowing the construction to achieve the optimal lower bound.

We first define the component-activating matrices and their role in updating the hidden state of the \hernnAcr{}.
% To construct the component-activating matrices more efficiently, 
In Indyk's construction, the component-activating matrices are based on \emph{four-hot} rather than two-hot encodings of states.
\begin{definition}
    Let $\wfsa = \fsatuple$ be an FSA, $\frNstates \defeq \ceil{\nstates^\frac{1}{4}}$, and $\perm$ a permutation of $\states = \NTo{\nstates}$.\footnote{The exact form of $\perm$ will be important later. For now, one can think of $\perm$ as the identity function.}
    We define the \defn{four-hot representation} of $\stateq \in \states$ as 
    \begin{equation}
        \phifour(\stateq) = \left(\ell_1, \ell_2, \ell_3, \ell_4\right)
    \end{equation}
    where 
    \begin{equation}
        \ell_\idxj = \frac{\perm\left(\stateq\right)}{\frNstates^{\idxj - 1}} \mod \frNstates.
    \end{equation}
    We denote the inverse of $\phifour$ with $\phifourInv$ and further define for $k \in \Zmod{\frNstates}$
    \begin{equation}
        % \phifourInvFun{k, \cdot, \cdot, \cdot} \defeq \set{\stateq \in \states \mid \evvarphi_0 = k; \phiCoor = \phifourFun{\stateq}}
        \phifourInvFun{k, \cdot, \cdot, \cdot} \defeq \set{\stateq \in \states \mid \phifourFun{\stateq}_1 = k}
    \end{equation}
    and $\phifourInvFun{\cdot, k, \cdot, \cdot}$, $\phifourInvFun{\cdot, \cdot, k, \cdot}$, and $\phifourInvFun{\cdot, \cdot, \cdot, k}$ analogously.
\end{definition}
We will denote $\phifourInvFun{\ldots, \idxk, \ldots}$ with $\idxk$ in $\idxj\textsuperscript{th}$  position (with $\idxj \in \Zmod{4}$) as $\compMtx{\idxk}{\idxj}$.
% Again, we assume that $\stateq \in \left\{0, \ldots, \nstates - 1\right\}$.
Despite using the four-hot representations, Indyk's construction still requires the two-hot representations based on $\phitwo$ as before.
In this case, however, they again depend on the chosen permutation $\perm$.
This allows us to define the component-activating matrices as follows.
\begin{definition}
    A \defn{component-activating matrix} in Indyk's construction is the representation matrix $\qMtx{\qPreds{\compMtx{\idxk}{\idxj}, \sym}}$ for some $\idxk \in \Zmod{\frNstates}$, $\idxj \in \Zmod{4}$, and $\sym \in \alphabet$.
\end{definition}
For efficient detection, the component-activating matrices are covered by so-called non-decreasing matrices.
\begin{definition}
    We say that $\mB \in \BDD$ is \defn{non-decreasing} if there exists a \emph{non-decreasing} (partial) function $\func\colon \Zmod{D} \to \Zmod{D}$ (from columns to rows) such that 
    \begin{equation}
        \mB_{\idxi \idxj} = 1 \iff \func\left(\idxj\right) = \idxi
    \end{equation}
    \textbf{and}, if $\func$ is defined for some $\idxj \in \Zmod{D}$, it is also defined for all $\idxj' \geq \idxj$.
\end{definition}
\begin{example}    
An example of a non-decreasing matrix is 
\begin{equation}
    \mB = \begin{pmatrix}
        0 & 1 & 0 & 0 \\
        0 & 0 & 0 & 0 \\
        0 & 0 & 1 & 1 \\
        0 & 0 & 0 & 0
    \end{pmatrix}.
\end{equation}
The function $\func$ defining the non-decreasing matrix $\mB$ is $\func = \begin{pmatrix}
    0 & 1 & 2 & 3 \\
    \emptyset & 0 & 1 & 1
\end{pmatrix}$, where $\emptyset$ denotes that the function is not defined.
\end{example}
Again, clearly, any matrix $\mB \in \BDD$ can be (non-uniquely) decomposed into at most $D$ non-decreasing matrices.
Moreover, non-decreasing matrices are detectable.
\begin{lemma}
    Non-decreasing matrices are detectable.
\end{lemma}
\begin{proof}
    Let $\mB \in \BDD$ be a non-decreasing matrix defined by the partial function $\func$.
    Divide the domain of $\func$ into the set of intervals in which the function is constant, with $I(\idxj)$ denoting the interval of $\idxj \in \Zmod{\frNstates^2}$ for $\idxj$ such that $\func\left(\idxj\right)$ is defined.
    Then, it is easy to see that $\emB_{\idxi \idxj} = 1 \iff \idxi = \func\left(\idxj\right)$, meaning that by defining the parameters $\vw$ and $b$ as 
    % \begin{align}
    %     \evw_{\idxj} &\defeq I(\idxj) \\
    %     \evw_{\frNstates^2 - 1 + \func\left(\idxj\right)} &\defeq \frNstates^2 - I\left(\idxj\right) \\
    %     b &\defeq -\frNstates^2
    %     % \vw \defeq \begin{pmatrix}
    %     %     I(0) & \ldots & I(\frNstates^2 - 1) & \mid & 
    %     % \end{pmatrix}
    % \end{align}
    \begin{align}
        \evw_{\func\left(\idxj\right)} &\defeq \frNstates^2 - I\left(\idxj\right) \\
        \evw_{\frNstates^2 + \idxj} &\defeq I(\idxj) \\
        b &\defeq -\frNstates^2
    \end{align}
    and other elements as $0$, we get that 
    \begin{equation} \label{eq:indyk-equality}
        % \emB_{\idxi \idxj} = 1 \iff I\left(\idxj\right) + \func\left(\idxj\right)
        \emB_{\idxi \idxj} = 1 \iff \idxi = \func\left(\idxj\right) \iff \evw_\idxi + \evw_\idxj + b = 0.
    \end{equation}
    % Recall that in the two-hot vector representation of a state (cf. \cref{def:vector-matrix-state-representation}), the entries $0, \ldots, \frNstates^2 - 1$ index the rows of the matrix state representation while the entries $\frNstates^2, \ldots, 2 \frNstates^2 - 1$ index the columns of the representation matrix.
    
    Compared to earlier, where component-activating matrices were detected by testing an \emph{inequality}, detecting a non-decreasing matrix requires testing an \emph{equality}.
    Since all terms in the equality are integers, testing the equality can be performed with the Heaviside activation function by conjoining two neurons; one testing the inequality $\evw_\idxi + \evw_\idxj + b - 1 < 0$ and another one testing the inequality $\evw_\idxi + \evw_\idxj + b + 1 > 0$.
    Both can individually be performed by a single neuron and then conjoined by an additional one.
\end{proof}
% The core idea behind Indyk's construction is a provably more efficient way of \emph{selecting} and \emph{decomposing} the parent matrices from Dewdney's construction.
% As we will see, other parts of the simulation are shared with Dewdney's construction.
% Note that, when decomposing a given binary matrix $\mB$ into non-decreasing matrices, one can first 
With this, the high-level idea of Indyk's construction is outlined in \cref{fig:indyk-high-level}.
After constructing the component-activating matrices based on $\phifour$ and decomposing them into non-decreasing matrices, the rest of Indyk's construction is very similar to Dewdney's construction, although the full update step of the \hernnAcr{} requires some additional processing.
To test the equality needed to detect non-decreasing matrices in the decomposition, \cref{eq:indyk-equality}, the four-hot representations are first converted into two-hot ones.
This can be done by a simple conjunction of the first two and the last two components of the four-hot representation.
Then, the activations of the non-decreasing matrices can be computed and disjoined into the representations of the component-activating matrices.
These form the $4 \nsymbols \frNstates$ components of the data sub-vector of the \hernnAcr{} hidden state.
They contain the activations of all possible next states, i.e., the children of the current state of $\wfsa$.
These are then conjoined with the representation of the current input symbol in the same way as in Dewdney's construction but adapted to the four-hot representations of the states.
The process is thus very similar to the phases of Dewdeney's construction illustrated in \cref{fig:dewdney-phases}.

Indyk's construction can be summarized by the following lemma.
\begin{lemma} \label{lemma:indyk-correct}
    Let $\wfsa = \fsatuple$ be a deterministic FSA.
    Then, Indyk's construction results in a \hernnAcr{} correctly simulating $\wfsa$'s transition function, i.e, $\hToQFun{\hiddStatet} = \qt$ for all $\tstep$.
\end{lemma}
\begin{proof}
Again, the proof follows the reasoning outlined above, and, to formally prove it is correct, we would have to follow a similar set of steps to how the correctness of Minsky's construction (\cref{lem:minsky-transitions}) was proved. We omit this for conciseness.
\end{proof}

The only remaining thing to show is that Indyk's construction achieves the theoretically optimal lower bound on the size of the \hernnAcr{} simulating a deterministic FSA.
All previous steps of the construction were valid no matter the chosen permutation $\perm$. 
The permutation, however, matters for space efficiency: Intuitively, it determines how efficiently one can decompose the resulting component-activating matrices (which depend on the permutation) into non-decreasing matrices in the sense of how many non-decreasing matrices are required to cover it.
Indyk, therefore, proved that there always exists, with non-zero probability, a permutation in which the decomposition across all states is efficient enough to achieve the minimum number of neurons required.
This is formalized by the following lemma.
\begin{lemma} \label{lemma:indyk-bound}
    Let $\wfsa = \fsatuple$ be a deterministic FSA.
    There exists a permutation of $\states$ such that Indyk's construction results in a \hernnAcr{} of size $\bigO{\nsymbols \sqrt{\nstates}}$.
\end{lemma}
\begin{proof}
    The proof can be found in \citet[][Lemma 6]{Indyk95}.
\end{proof}
% \begin{proof}
%     The proof can be found in \citet{Indyk95}.
% \end{proof}
This concludes our presentation of Indyk's construction.
All results stated in this section can be summarized by the following theorem.
\begin{theorem}
    Let $\wfsa = \fsatuple$ be a deterministic FSA.
    There exists a \hernnAcr{} of size $\bigO{\nsymbols \sqrt{\nstates}}$ correctly simulating $\wfsa$.
\end{theorem}
\begin{proof}
Again, the proof follows from the fact that Indyk's construction correctly simulates the FSA (cf. \cref{lemma:indyk-correct}) while the space bound is guaranteed by \cref{lemma:indyk-bound}.
\end{proof}

% \begin{align}
% \vh_{\project[1]} &= \bigvee_{(\iota_1, \iota_2)} \left( \vh_{\iota_1} \land \vh_{\iota_2}\right)
% \end{align}

% \begin{figure}
%     \centering
%     \begin{tikzpicture}
%       \matrix[matrix of math nodes, column sep=1cm, row sep=1cm, nodes={minimum width=1.5cm}] (mat) {
%         \begin{pmatrix}
%           v_{11} \\ v_{12} \\ v_{13} \\ v_{14} \\ v_{15}
%         \end{pmatrix} &
%         \begin{pmatrix}
%           v_{21} \\ v_{22} \\ v_{23} \\ v_{24} \\ v_{25}
%         \end{pmatrix} &
%         \begin{pmatrix}
%           v_{31} \\ v_{32} \\ v_{33} \\ v_{34} \\ v_{35}
%         \end{pmatrix} &
%         \begin{pmatrix}
%           v_{41} \\ v_{42} \\ v_{43} \\ v_{44} \\ v_{45}
%         \end{pmatrix} &
%         \begin{pmatrix}
%           v_{51} \\ v_{52} \\ v_{53} \\ v_{54} \\ v_{55}
%         \end{pmatrix} \\
%       };
%       \foreach \i in {1,...,5} {
%         \node at ([yshift=0.25cm]mat-1-\i.north) {\small Phase \i};
%       }
%       \foreach \i in {1,...,4} {
%         \draw [->,thick] (mat-1-\i.east) -- (mat-1-\the\numexpr\i+1\relax.west);
%       }
%     \end{tikzpicture}
%     \caption{A high-level illustration of how the transition function of the FSA is implemented by 5 applications of the Elman update rule.}
%     \label{fig:indyk-high-level}
% \end{figure}


\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/Indyk.pdf}
    \caption{High-level overview of Indyk's construction. 
    The highlighted \textcolor{ETHBronze}{orange} neuron in the representation of the state from the data sub-vector corresponds to the activation of one of the components of the \textcolor{ETHRed}{red} states (which have in common that their $0\textsuperscript{th}$ component of $\phifourFun{\stateq}$ is the same). 
    The matrix corresponding to the disjunction of the representations of their \emph{$\sym$-parents} (\textcolor{ETHBlue}{blue} states) is decomposed into two non-decreasing matrices. 
    The non-zero elements of both can be detected by a conjunction of two neurons; here, $\func_1 = \begin{pmatrix}
        0 & 1 & 2 & 3 \\
        \emptyset & 0 & 0 & 0
    \end{pmatrix}$ and $\func_2 = \begin{pmatrix}
        0 & 1 & 2 & 3 \\
        \emptyset & \emptyset & 1 & 2
    \end{pmatrix}$, meaning that $\vw_1 = \begin{pmatrix}
        3 & 0 & 0 & 0 & \mid & 0 & 1 & 1 & 1
    \end{pmatrix}$, $\vw_2 = \begin{pmatrix}
        0 & 3 & 2 & 0 & \mid & 0 & 0 & 1 & 2
    \end{pmatrix}$, and $b_1 = b_2 = 4$.
    Those activations are then disjoined to result in the activation in the \textcolor{ETHBronze}{orange} neuron.
    The \textcolor{ETHPurple}{purple} neurons in the processing sub-vector are composed of the neurons in the networks implementing the detection of line matrices and their conjunctions and disjunctions (also shown in \textcolor{ETHPurple}{purple}).
    Note that even if the second matrix were not non-decreasing in itself (i.e., the columns of the two ones would be flipped), one could still transform it into a non-decreasing matrix by permuting the columns and permuting the corresponding neurons.}
    \label{fig:indyk-high-level}
\end{figure*}


% \begin{figure*}
%     \centering
%     \begin{tikzpicture}
%       \matrix[matrix of math nodes, column sep=0.6cm, row sep=5mm, nodes={minimum width=1.5cm}] (mat) {
%         \begin{tikzpicture}[node distance = 6mm]
%         \tiny
%         \node[state, fill=ETHPurple!30, draw=ETHPurple!80] (q){ $\stateq$ }; 
%         \node[state] (q1) [above right = of q] { $\stateq'$ }; 
%         \node[state] (q2) [below right = of q] { $\stateq''$ }; 
%         \draw (q) edge[above, sloped] node{ $\syma$ } (q1) 
%         (q) edge[above, sloped] node{ $\symb$ } (q2);
%         \end{tikzpicture} & 
%         \begin{tikzpicture}[node distance = 6mm]
%         \tiny
%         \node[state, fill=ETHPurple!30, draw=ETHPurple!80] (q){ $\stateq$ }; 
%         \node[state] (q1) [above right = of q] { $\stateq'$ }; 
%         \node[state] (q2) [below right = of q] { $\stateq''$ }; 
%         \draw (q) edge[above, sloped] node{ $\syma$ } (q1) 
%         (q) edge[above, sloped] node{ $\symb$ } (q2);
%         \end{tikzpicture}
%         &
%         \begin{tikzpicture}[node distance = 6mm]
%         \tiny
%         \node[state] (q){ $\stateq$ }; 
%         \node[state, fill=ETHPetrol!20] (q1) [above right = of q] { $\stateq'$ }; 
%         \node[state, fill=ETHPetrol!20] (q2) [below right = of q] { $\stateq''$ }; 
%         \draw (q) edge[ETHPetrol, above, sloped] node{ $\syma$ } (q1) 
%         (q) edge[ETHPetrol, above, sloped] node{ $\symb$ } (q2);
%         \end{tikzpicture} &
%         \begin{tikzpicture}[node distance = 6mm]
%         \tiny
%         \node[state] (q){ $\stateq$ }; 
%         \node[state, fill=ETHGreen!30, draw=ETHGreen!80] (q1) [above right = of q] { $\stateq'$ }; 
%         \node[state] (q2) [below right = of q] { $\stateq''$ }; 
%         \draw (q) edge[ETHGreen, above, sloped] node{ $\syma$ } (q1) 
%         (q) edge[above, sloped] node{ $\symb$ } (q2);
%         \end{tikzpicture} &
%         \begin{tikzpicture}[node distance = 6mm]
%         \tiny
%         \node[state] (q){ $\stateq$ }; 
%         \node[state, fill=ETHGreen!30, draw=ETHGreen!80] (q1) [above right = of q] { $\stateq'$ }; 
%         \node[state] (q2) [below right = of q] { $\stateq''$ }; 
%         \draw (q) edge[ETHGreen, above, sloped] node{ $\syma$ } (q1) 
%         (q) edge[above, sloped] node{ $\symb$ } (q2);
%         \end{tikzpicture} \\
%         \begin{pmatrix}
%           \vu_{1} \\ \vu_{2} \\ \vu_{3} \\ \vu_{4}
%         \end{pmatrix} &
%         \begin{pmatrix}
%           \vv_{1} \\ \vv_{2}
%         \end{pmatrix} &
%         \begin{pmatrix}
%           v_{31} \\ v_{32} \\ v_{33} \\ v_{34}
%         \end{pmatrix} &
%         \begin{pmatrix}
%           v_{41} \\ v_{42} \\ v_{43} \\ v_{44}
%         \end{pmatrix} &
%         \begin{pmatrix}
%           \vu_{1}' \\ \vu_{2}' \\ \vu_{3}' \\ \vu_{4}'
%         \end{pmatrix} \\
%       };
      
      
%       \foreach \i in {1,...,5} {
%         \node at ([yshift=0.25cm]mat-2-\i.north) {\small Phase \i};
%       }
      
%       \node at ([yshift=-0.25cm]mat-2-1.south) {\small $4r$};
%       \node at ([yshift=-0.25cm]mat-2-2.south) {\small $2r^2$};
%       \node at ([yshift=-0.25cm]mat-2-3.south) {\small $4r\nfs|\eosalphabet|$};
%       \node at ([yshift=-0.25cm]mat-2-4.south) {\small $4r\nfs|\eosalphabet|$};
%       \node at ([yshift=-0.25cm]mat-2-5.south) {\small $4r$};
      
%       \foreach \i in {1,...,4} {
%         \draw [->,thick] (mat-2-\i.east) -- (mat-2-\the\numexpr\i+1\relax.west);
%       }
%     \end{tikzpicture}
%     \caption{A high-level illustration of how the transition function of the FSA is implemented by 5 applications of the Elman update rule.}
%     \label{fig:indyk-high-level}
% \end{figure*}


% \begin{figure*}
%     \centering
%     \begin{tikzpicture}
%       \matrix[matrix of math nodes, column sep=0.6cm, row sep=0.5cm, nodes={minimum width=1.5cm}] (mat) {
%         % \begin{tikzpicture}[node distance = 6mm]
%         % \tiny
%         % \node[state] (q1){ $\stateq_1$ }; 
%         % \node[state] (q2) [below = of q1] { $\stateq_2$ }; 
%         % \node[state] (q3) [below = of q2] { $\stateq_3$ }; 
%         % \node[state] (q4) [below = of q3] { $\stateq_4$ }; 
%         % \node[state] (q5) [right = of q1, yshift=-5mm] { $\stateq_5$ }; 
%         % \node[state] (q6) [right = of q2, yshift=-5mm] { $\stateq_6$ }; 
%         % \node[state] (q7) [right = of q3, yshift=-5mm] { $\stateq_7$ }; 
%         % \draw (q1) edge[above, sloped] node{ $\syma$ } (q5) 
%         % (q1) edge[above, sloped] node{ $\syma$ } (q6) 
%         % (q2) edge[above, sloped] node{ $\syma$ } (q5) 
%         % (q2) edge[above, sloped] node{ $\syma$ } (q6) 
%         % (q3) edge[above, sloped] node{ $\syma$ } (q7) 
%         % (q4) edge[above, sloped] node{ $\syma$ } (q6) 
%         % (q4) edge[above, sloped] node{ $\syma$ } (q7) ;
%         % \end{tikzpicture}
%         \begin{tikzpicture}[node distance = 4mm]
%         \tiny
%         \node[state] (q1){ $\stateq_1$ }; 
%         \node[state] (q2) [below = of q1] { $\stateq_2$ }; 
%         \node[state] (q3) [below = of q2] { $\stateq_3$ }; 
%         \node[state] (q4) [right = of q1, yshift=-5mm, fill=ETHRed!30, draw=ETHRed!80] { $\stateq_4$ }; 
%         \node[state] (q5) [right = of q2, yshift=-5mm, fill=ETHRed!30, draw=ETHRed!80] { $\stateq_5$ }; 
%         \draw (q1) edge[above, sloped] node{ $\syma$ } (q4) 
%         (q2) edge[above, sloped] node{ $\syma$ } (q4) 
%         (q3) edge[above, sloped] node{ $\syma$ } (q5) ;
%         \end{tikzpicture} & 
%         \begin{tikzpicture}[node distance = 4mm]
%         \tiny
%         \node[state] (q1) [draw=ETHGreen!80, fill=ETHGreen!30] { $\stateq_1$ }; 
%         \node[state] (q2) [below = of q1, draw=ETHGreen!80, fill=ETHGreen!30] { $\stateq_2$ }; 
%         \node[state] (q3) [below = of q2, draw=ETHGreen!80, fill=ETHGreen!30] { $\stateq_3$ }; 
%         \node[state] (q4) [right = of q1, yshift=-5mm] { $\stateq_4$ }; 
%         \node[state] (q5) [right = of q2, yshift=-5mm] { $\stateq_5$ }; 
%         \draw (q1) edge[above, sloped] node{ $\syma$ } (q4) 
%         (q2) edge[above, sloped] node{ $\syma$ } (q4) 
%         (q3) edge[above, sloped] node{ $\syma$ } (q5) ;
%         \end{tikzpicture}
%         &
%         \begin{tikzpicture}[node distance = 4mm]
%         \tiny
%         \node[state] (q1) { $\stateq_1$ }; 
%         \node[state] (q2) [below = of q1, draw=ETHGreen!80, fill=ETHGreen!30] { $\stateq_2$ }; 
%         \node[state] (q3) [below = of q2, draw=ETHGreen!80, fill=ETHGreen!30] { $\stateq_3$ }; 
%         \node[state] (q4) [right = of q1, yshift=-5mm] { $\stateq_4$ }; 
%         \node[state] (q5) [right = of q2, yshift=-5mm] { $\stateq_5$ }; 
%         \draw (q1) edge[above, sloped] node{ $\syma$ } (q4) 
%         (q2) edge[above, sloped] node{ $\syma$ } (q4) 
%         (q3) edge[above, sloped] node{ $\syma$ } (q5) ;
%         \end{tikzpicture}
%         &
%         \begin{tikzpicture}[node distance = 4mm]
%         \tiny
%         \node[state] (q1) [draw=ETHGreen!80, fill=ETHGreen!30] { $\stateq_1$ }; 
%         \node[state] (q2) [below = of q1] { $\stateq_2$ }; 
%         \node[state] (q3) [below = of q2] { $\stateq_3$ }; 
%         \node[state] (q4) [right = of q1, yshift=-5mm] { $\stateq_4$ }; 
%         \node[state] (q5) [right = of q2, yshift=-5mm] { $\stateq_5$ }; 
%         \draw (q1) edge[above, sloped] node{ $\syma$ } (q4) 
%         (q2) edge[above, sloped] node{ $\syma$ } (q4) 
%         (q3) edge[above, sloped] node{ $\syma$ } (q5) ;
%         \end{tikzpicture}
%         &
%         \begin{tikzpicture}[node distance = 6mm]
%         \tiny
%         \node[state] (q){ $\stateq$ }; 
%         \node[state, fill=ETHGreen!30, draw=ETHGreen!80] (q1) [above right = of q] { $\stateq'$ }; 
%         \node[state] (q2) [below right = of q] { $\stateq''$ }; 
%         \draw (q) edge[ETHGreen, above, sloped] node{ $\syma$ } (q1) 
%         (q) edge[above, sloped] node{ $\symb$ } (q2);
%         \end{tikzpicture} \\
%          &
%         \begin{pmatrix}
%             & 1 & \\
%             & 1 & 1 \\
%             & & 
%         \end{pmatrix} =  &
%         \begin{pmatrix}
%             & 1 & \\
%             & & 1 \\
%             & & 
%         \end{pmatrix} +  &
%         \begin{pmatrix}
%             &  & \\
%             & 1 &  \\
%             & & 
%         \end{pmatrix} &
%         \begin{pmatrix}
%           \vu_{1}' \\ \vu_{2}' \\ \vu_{3}' \\ \vu_{4}'
%         \end{pmatrix} \\
%       };
      
%     \end{tikzpicture}
%     \caption{A high-level illustration of how the non-decreasing matrices detecting the activations of the next states are constructed. Here, we have $\sA \defeq \phifourInvFun{0, *, *, *} = \set{\textcolor{ETHRed}{\stateq_4, \stateq_5}}$. Further, we have $\phitwoFun{\stateq_1} = \left(1, 1\right)$, $\phitwoFun{\stateq_2} = \left(2, 1\right)$, and $\phitwoFun{\stateq_3} = \left(1, 0\right)$.}
%     \label{fig:indyk-high-level-construction}
% \end{figure*}


% \begin{figure*}
%     \centering
%     \begin{tikzpicture}
%         \node[align=center] (setA) {
%             \begin{tikzpicture}[node distance = 4mm]
%             \tiny
%             \node[state] (q1){ $\stateq_1$ }; 
%             \node[state] (q2) [below = of q1] { $\stateq_2$ }; 
%             \node[state] (q3) [below = of q2] { $\stateq_3$ }; 
%             \node[state] (q4) [right = of q1, yshift=-5mm, fill=ETHRed!30, draw=ETHRed!80] { $\stateq_4$ }; 
%             \node[state] (q5) [right = of q2, yshift=-5mm, fill=ETHRed!30, draw=ETHRed!80] { $\stateq_5$ }; 
%             \draw (q1) edge[above, sloped] node{ $\syma$ } (q4) 
%             (q2) edge[above, sloped] node{ $\syma$ } (q4) 
%             (q3) edge[above, sloped] node{ $\syma$ } (q5) ;
%             \end{tikzpicture}
%         };
%         \node[align=center, right = of setA] (predA) {
%             \begin{tikzpicture}[node distance = 4mm]
%             \tiny
%             \node[state] (q1) [draw=ETHGreen!80, fill=ETHGreen!30] { $\stateq_1$ }; 
%             \node[state] (q2) [below = of q1, draw=ETHGreen!80, fill=ETHGreen!30] { $\stateq_2$ }; 
%             \node[state] (q3) [below = of q2, draw=ETHGreen!80, fill=ETHGreen!30] { $\stateq_3$ }; 
%             \node[state] (q4) [right = of q1, yshift=-5mm] { $\stateq_4$ }; 
%             \node[state] (q5) [right = of q2, yshift=-5mm] { $\stateq_5$ }; 
%             \draw (q1) edge[above, sloped] node{ $\syma$ } (q4) 
%             (q2) edge[above, sloped] node{ $\syma$ } (q4) 
%             (q3) edge[above, sloped] node{ $\syma$ } (q5) ;
%             \end{tikzpicture}
%         };
%         \node[align=center, below = of predA] (predM) {
%             $\begin{pmatrix}
%                 & 1 & \\
%                 & & 1 \\
%                 & & 1
%             \end{pmatrix}$
%         };
%         \node[align=center, right = of predM, xshift=2cm, yshift=1cm] (predM1) {
%             $\begin{pmatrix}
%                 & 1 & \\
%                 & & 1 \\
%                 & & 
%             \end{pmatrix}$
%         };
%         \node[align=center, right = of predM, xshift=2cm, yshift=-1cm] (predM2) {
%             $\begin{pmatrix}
%                 & & \\
%                 & \phantom{1} & \\
%                 & & 1
%             \end{pmatrix}$
%         };
%         \draw [->,thick] (predM.east) -- (predM1.west);
%         \draw [->,thick] (predM.east) -- (predM2.west);
%         \node[align=center, above = of predM1] (predA1) {
%             \begin{tikzpicture}[node distance = 4mm]
%             \tiny
%             \node[state] (q1) { $\stateq_1$ }; 
%             \node[state] (q2) [below = of q1, draw=ETHGreen!80, fill=ETHGreen!30] { $\stateq_2$ }; 
%             \node[state] (q3) [below = of q2, draw=ETHGreen!80, fill=ETHGreen!30] { $\stateq_3$ }; 
%             \node[state] (q4) [right = of q1, yshift=-5mm] { $\stateq_4$ }; 
%             \node[state] (q5) [right = of q2, yshift=-5mm] { $\stateq_5$ }; 
%             \draw (q1) edge[above, sloped] node{ $\syma$ } (q4) 
%             (q2) edge[above, sloped] node{ $\syma$ } (q4) 
%             (q3) edge[above, sloped] node{ $\syma$ } (q5) ;
%             \end{tikzpicture}
%         };
%         \node[align=center, below = of predM2] (predA2) {
%             \begin{tikzpicture}[node distance = 4mm]
%             \tiny
%             \node[state] (q1) [draw=ETHGreen!80, fill=ETHGreen!30] { $\stateq_1$ }; 
%             \node[state] (q2) [below = of q1] { $\stateq_2$ }; 
%             \node[state] (q3) [below = of q2] { $\stateq_3$ }; 
%             \node[state] (q4) [right = of q1, yshift=-5mm] { $\stateq_4$ }; 
%             \node[state] (q5) [right = of q2, yshift=-5mm] { $\stateq_5$ }; 
%             \draw (q1) edge[above, sloped] node{ $\syma$ } (q4) 
%             (q2) edge[above, sloped] node{ $\syma$ } (q4) 
%             (q3) edge[above, sloped] node{ $\syma$ } (q5) ;
%             \end{tikzpicture}
%         };
%         \node[align=center, right = of predM1] (f1) {
%             $\func_1 = \begin{pmatrix}
%                 1 & 2 & 3 \\
%                 \emptyset & 1 & 2
%             \end{pmatrix}$ \\
%             $\vw_1 = \begin{pmatrix} 3 & 2 & 0 \mid 0 & 1 & 2 \end{pmatrix}$
%         };
%         \node[align=center, right = of predM2] (f2) {
%             $\func_1 = \begin{pmatrix}
%                 1 & 2 & 3 \\
%                 \emptyset & \emptyset & 3
%             \end{pmatrix}$ \\
%             $\vw_2 = \begin{pmatrix} 0 & 0 & 3 \mid 0 & 0 & 1 \end{pmatrix}$
%         };
%     \end{tikzpicture}
%     \caption{A high-level illustration of how the non-decreasing matrices detecting the activations of the next states are constructed. Here, we have $\sA \defeq \phifourInvFun{0, *, *, *} = \set{\textcolor{ETHRed}{\stateq_4, \stateq_5}}$. Further, we have $\phitwoFun{\stateq_1} = \left(2, 2\right)$, $\phitwoFun{\stateq_2} = \left(2, 1\right)$, and $\phitwoFun{\stateq_3} = \left(1, 0\right)$.
%     Note that the fact that $\mB_\sA$ decomposes into two non-deceasing matrices is a not necessary---usually, a permutation of the columns would be needed.}
%     \label{fig:indyk-high-level-construction}
% \end{figure*}

% \subsection{Generalizing Weighted Case}
% {
% \color{ETHRed}
% \begin{itemize}
%     \item We can't go smaller than linear in altogether
%     \item We can augment the efficient constructions with the mapping from the multi-hot representations to the one-hot representation using a simple MLP (conjunction)
%     \item This correctly matches the probabilities but does not improve the asymptotic complexity.
% \end{itemize}
% }

==> sections/equivalence.tex <==
The hidden states of an \hernnAcr{} live in $\B^\hiddDim$, and can thus take $2^\hiddDim$ different values.
This inspires the interpretation of $\hiddState$ as the state of an underlying FSA that transitions between states based on the \hernnAcr{} update rule, specifying its local conditional distributions with the output matrix $\outMtx$. 
% This is the main idea behind the proof that \hernnAcr{}s characterize finite-state LMs.
On the other hand, one can also imagine designing a \hernnAcr{} that simulates the transitions of a given FSA by appropriately specifying the parameters of the \hernnAcr{}.
We explore this connection formally in this section and present the main technical result of the paper.
The central result that characterizes the expressive capacity \hernnAcr{} can be informally summarized by the following theorem.
\begin{theorem}[Informal] \label{thm:elman-pfsa-euqivalent}
    \hernnAcr{} LMs are equivalent to \dpfsaAcr{}s.
\end{theorem}
We split this result into the question of \textit{(i)} how \dpfsaAcr{}s can simulate \hernnAcr{} LMs and \textit{(ii)} how \hernnAcr{} LMs can simulate \dpfsaAcr{}s.
% We first show that \hernnAcr{}s are always finite-state, and then show how they can simulate any \dpfsaAcr{}.

\subsection{\dpfsaAcr{}s Can Simulate \hernnAcr{}s}
\begin{restatable}{reLemma}{hernnRegularLemma} \label{lem:heaviside-rnns-regular}
Let $\rnnlm$ be a \hernnAcr{} LM defining the LM $\pLN$. 
Then, there exists a \dpfsaAcr{} $\wfsa$ such that $\wfsa\left(\str\right) = \pLN\left(\str\right)$ for every $\str \in \kleene{\alphabet}$.
% The distribution represented by a recurrent neural network with a Heaviside nonlinearity $\heaviside$ is regular.
\end{restatable}
The proof closely follows the intuitive reasoning outlined above and is presented in \cref{app:proofs}.
This implies that \hernnAcr{}s are at most as expressive as \dpfsaAcr{}s, and as a consequence, strictly less expressive as non-deterministic PFSAs.
We discuss the implications of this result later in \cref{sec:discussion}.

==> sections/fslms.tex <==
% \begin{figure}[t]
%     \centering
%     % \footnotesize
%     \begin{tikzpicture}[node distance=8mm, minimum size=12mm]
%         % \footnotesize
%         \node[state, initial] (q0) [] { $\scriptstyle \stateq_0/\textcolor{ETHGreen}{1}$ }; 
%         \node[state] (q1) [above right = of q0, xshift=13mm, yshift=-3mm] { $\scriptstyle \stateq_1$ }; 
%         \node[state, accepting] (q2) [below right = of q0, xshift=12mm, yshift=3mm] { $\scriptstyle \stateq_2/\textcolor{ETHRed}{0.3}$ }; 
%         \draw[transition] (q0) edge[auto, bend left, sloped] node[minimum size=4mm]{ $\syma/{\scriptstyle 0.6}$ } (q1) 
%         (q0) edge[auto, bend right, sloped] node[minimum size=4mm]{ $\symb/{\scriptstyle 0.4}$ } (q2)
%         (q1) edge[auto, loop right] node[minimum size=4mm]{ $\symb/{\scriptstyle 0.1}$ } (q1)
%         (q1) edge[auto] node[minimum size=4mm]{ $\syma/{\scriptstyle 0.9}$ } (q2)
%         (q2) edge[auto, loop right] node[minimum size=4mm]{ $\symb/{\scriptstyle 0.7}$ } (q2) ;
%     \end{tikzpicture}
%     \begin{tabular}{ll}
%             % $\pdens(\syma \mid \stateq_0)$ & 0.5 \\
%             % $\pdens(\symb \mid \stateq_0)$ & 0.5 \\
%             % $\pdens(\syma \mid \stateq_1)$ & 0.9 \\
%             % $\pdens(\symb \mid \stateq_1)$ & 0.1 \\
%             % $\pdens(\symb \mid \stateq_1)$ & 0.5 \\
%             % $\pdens(\eos \mid \stateq_1)$ & 0.5 \\
%             % \midrule \\
%             % $\pdens(\syma)$ & $0$ \\
%             \normalsize $\pdens(\syma \symb^n \syma \symb^m)\colon$ & \normalsize $\textcolor{ETHGreen}{1} \cdot 0.6 \cdot 0.1^n \cdot 0.9 \cdot 0.7^m \cdot \textcolor{ETHRed}{0.3}$ \\
%             \normalsize $\pdens(\symb \symb^m)\colon$ & \normalsize $\textcolor{ETHGreen}{1} \cdot 0.4 \cdot 0.7^m \cdot \textcolor{ETHRed}{0.3}$
%             % $\pdens(\symb)$ & $0.5 \cdot 0.5 = 0.25$ \\
%             % $\pdens(\syma \symb)$ & $0.5 \cdot 0.9 \cdot 0.5 = 0.225$
%     \end{tabular}  
%     \caption{A weighted finite-state automaton defining a probability distribution over $\kleene{\set{\syma, \symb}}$.}
%     \label{fig:example-fslm}
% \end{figure}

Most modern LMs define $\pLM\left(\str\right)$ as a product of conditional probability distributions $\pLNSM$:
\begin{equation} \label{eq:lnlm}
    \pLN\left(\str\right) \defeq \pLNSM\left(\eos\mid\str\right) \prod_{\tstep = 1}^{|\str|} \pLNSM\left(\symt \mid \strlt\right),
\end{equation}
where $\eos \notin \alphabet$ is a special \underline{e}nd \underline{o}f \underline{s}equence symbol, which enables defining probabilities of strings based on purely conditional distributions.
Such models are called locally normalized.
We denote $\eosalphabet \defeq \alphabet \cup \left\{\eos\right\}$.
% $\pLN$ may not define a language model: that is, it may not hold that $\sum_{\str\in \kleene{\alphabet}} \pLN(\str) = 1$.
% Models defining a valid distribution over $\kleene{\alphabet}$ tight. 
Throughout this paper, we will assume $\pLN$ defines a valid probability distribution over $\kleene{\alphabet}$, i.e., that $\pLN$ is tight \citep{du-etal-2023-measure}.
% We will refer to the string $\str$ in $\pLNSM\left(\sym \mid \str\right)$ as the \defn{context}.

% \subsection{Weighted Finite-state Automata} \label{sec:wfsa}
% \anej{I started putting in the definitions from LLM, but I'm not sure: should we just define PFSAs like in Leo's paper?}

Finite-state automata are a tidy and well-understood formalism for describing formal languages.
In words, they represent the simplest devices for defining a formal language.
% We give a formal definition below.
\begin{definition} \label{def:fsa}
    A \defn{finite-state automaton} (FSA) is a 5-tuple $\fsatuple$ where $\alphabet$ is an alphabet, $\states$ a finite set of states, $\initial, \final \subseteq \states$ the set of initial and final states, and $\trans \subseteq \states \times \alphabet \times \states$ set of transitions.
    % \anej{I left out $\eps$'s and constrained it to a set of transitions.}
    % Elements of $\trans$ are called \defn{transitions}. 
\end{definition}
We assume that states are identified by integers in $\Z_\nstates \defeq \set{0, \ldots, \nstates - 1}$.\footnote{For a cleaner presentation, we also assume that vectors and matrices are zero-indexed.}
% , i.e, $\states = \Z_{\pathlen + 1}$ for some $N$.
We also adopt a more suggestive notation for transitions by denoting $\left(\stateq, \sym, \stateq' \right) \in \trans$ as $\uwedge{\stateq}{\sym}{\stateq'}$ and call transitions of the form $\uwedge{\stateq}{\sym}{\stateq'}$ $\sym$-transitions.
Furthermore, we define $\qPreds{\stateq; \sym} \defeq \set{\stateq' \mid \exists \sym \in \alphabet\colon \uwedge{\stateq'}{\sym}{\stateq} \in \trans}$ as the set of $\sym$-parents of $\stateq$
% , i.e., states from which $\stateq$ can be reached by taking a $\sym$-transition 
and the \defn{children} of the state $\stateq$ as the set $\set{\stateq' \mid \exists \sym \in \alphabet\colon \uwedge{\stateq}{\sym}{\stateq'} \in \trans}$.\looseness=-1

% An FSA sequentially reads individual symbols of an input string $\str \in \kleene{\alphabet}$ and transitions between states according to the transition function $\trans$.
% The traversal through the automaton starts in a state $\qinit \in \initial$ and transitions from $\stateq$ into $\stateq'$ upon reading the symbol $\sym$ if and only if $\uwedge{\stateq}{\sym}{\stateq'} \in \trans$.
% In this sense, the current state $\stateq$ after reading in some prefix of the input string $\strlt$ can be seen as a compact (finite-space) summary of $\strlt$.

% A common augmentation of FSAs is the addition of weights.
FSAs are often augmented with weights.
\begin{definition}
A \defn{real-weighted finite-state automaton} (WFSA) $\automaton$ is a 5-tuple $\wfsatuple$ where $\alphabet$ is an alphabet, $\states$ a finite set of states, $\trans \subseteq \states \times \alphabet \times \R \times \states$ a finite set of weighted transitions and $\initf, \finalf\colon \states \rightarrow \R$ the initial and final weighting functions. 
\end{definition}
We denote $\left(\stateq, \sym, w, \stateq'\right) \in \trans$ with $\edge{\stateq}{\sym}{w}{\stateq'}$ and define $\transitionWeight(\edge{\stateq}{\sym}{w}{\stateq'}) \defeq w$, where $\transitionWeight(\edge{\stateq}{\sym}{\circ}{\stateq'}) \defeq 0$ if there are no $\sym$-transitions from $\stateq$ to $\stateq'$.\footnote{Throughout the text, we use $\circ$ as a placeholder a free quantity, in this case, to any weight $w \in \R$. In case there are multiple $\circ$'s in an expression, they are not tied in any way.}
% We omit the initial and final sets, which are defined implicitly by the states given non-zero initial or final weights, i.e., $\initial = \left\{\stateq \in \states \mid \initf\left(\stateq\right) \neq 0\right\}$ and $\final = \left\{\stateq \in \states \mid \finalf\left(\stateq\right) \neq 0\right\}$.
% We will refer to them for notational convenience.
The \defn{underlying FSA} of a WFSA is the FSA obtained by removing the transition weights and setting $\initial = \set{\stateq \in \states \mid \initfFun{\stateq}}$ and $\final = \set{\stateq \in \states \mid \finalfFun{\stateq}}$.
\begin{definition} \label{def:fsa-deterministic}
An FSA $\automaton = \fsatuple$ is \defn{deterministic} if $|\initial| = 1$ and for every $(\stateq, \sym) \in \states \times \alphabet$, there is at most one $\stateq' \in \states$ such that $\uwedge{\stateq}{\sym}{\stateq'} \in \trans$.
A WFSA is deterministic if its underlying FSA is deterministic.
% A WFSA $\automaton = \wfsatuple$ is deterministic if $|\set{\stateq \in \states \mid \initfFun{\stateq} \neq 0}| = 1$ and for every $(\stateq, \sym) \in \states \times \alphabet$, there is at most one $\stateq' \in \states$ such that $\edge{\stateq}{\sym}{w}{\stateq'} \in \trans$ for some $w \in \R$.
% Otherwise, $\automaton$ is \defn{non-deterministic}.
\end{definition}
% The definition can be generalized to the weighted case by requiring that $|\set{\stateq \in \states \mid \initfFun{\stateq}}| = 1$.
In contrast to unweighted FSAs, not all non-deterministic WFSAs admit an equivalent deterministic one (they are non-determinizable). 
% This has important implications for the relationship between the class of distributions defined by WFSAs and RNNs.

\begin{definition}
A \defn{path} $\apath$ is a sequence of consecutive transitions $\edge{\stateq_1}{\sym_1}{w_1}{\stateq_2}, \cdots, \edge{\stateq_{\pathlen}}{\sym_{\pathlen}}{w_{\pathlen}}{\stateq_{\pathlen + 1}}$.
Its \defn{length} $|\apath|$ is the number of transition in it and its \defn{scan} $\yield\left(\apath\right)$ the concatenation of the symbols on them. 
We denote with $\paths(\automaton)$ the set of all paths in $\automaton$ and with $\paths(\automaton, \str)$ the set of all paths that scan $\str \in \kleene{\alphabet}$.\looseness=-1
\end{definition} 
% Note that $|\paths\left(\automaton, \str\right)| = 1$ for all $\str \in \kleene{\alphabet}$ if $\wfsa$ is deterministic.

The weights of the transitions along a path are multiplicatively combined to form the weight of the path.
The weights of all the paths scanning the same string are combined additively to form the weights of that string.
\begin{definition}
The \defn{path weight} of $\apath$ is $\weight\left(\apath\right) = \initf \left( \stateq_1 \right) \left[\prod_{\idx = 1}^\pathlen w_\idx\right] \finalf \left( \stateq_{\pathlen + 1} \right)$.
% $\weight\left(\apath\right) = \initf \left( \prevq \left( \apath \right) \right) \left[\prod_{\idx = 1}^\pathlen w_\idx\right] \finalf \left( \nextq \left( \apath \right) \right)$.
% $\apath$ is \defn{accepting} if $\weight\left(\apath\right) \neq \zero$. 
% \end{definition}
% \begin{definition}

The \defn{stringsum} of $\str \in \kleene{\alphabet}$
% under a WFSA $\automaton$ 
is $\automaton \left( \str \right) \defeq \sum_{\apath \in \paths\left( \automaton, \str \right) }  \weight \left( \apath \right)$.
\end{definition}
% The stringsum naturally generalizes the acceptance by an unweighted FSA---whereas an unweighted FSA only makes a binary decision of accepting or rejecting a string, a weighted FSA accepts a string with a specific weight.

% We will use WFSAs to specify LMs.
% However, not every WFSA is an LM, i.e., a distribution over strings.
A class of WFSAs important for defining LMs is probabilistic WFSAs.
\begin{definition}\label{def:stochastic-wfsa}
A WFSA $\wfsa = \wfsatuple$ is \defn{probabilistic} (a PFSA) if all transition, initial, and final weights are non-negative, $\sum_{\stateq \in \states} \initf\left(\stateq\right) = 1$, and, for all $\stateq \in \states$, $\sum_{\edge{\stateq}{\sym}{w}{\stateq'} \in \trans} w + \finalf\left(\stateq\right) = 1$.
\end{definition}
The initial weights, 
% (the initial weight of a state corresponds to the \emph{probability} of starting in it), 
and, for any $\stateq \in \states$, the weights of its outgoing transitions and its final weight, form a probability distribution.
The final weights in a PFSA play an analogous role to the $\eos$ symbol---they represent the probability of ending a path in $\stateq$: $\finalf\left(\stateq\right)$ corresponds to the probability of ending a string $\str$, $\pLNSM\left(\eos \mid \str\right)$, where $\stateq$ is a state arrived at by $\wfsa$ after reading $\str$.
% When drawing the connection between LMs and PFSAs, we will specify $\pLNSM\left(\eos \mid \str\right)$ in terms of the final weights $\finalf$.
We will use the acronym \dpfsaAcr{} for the important special case of a deterministic PFSA. 
\begin{figure}[t]
    \centering
    % \footnotesize
    \begin{tikzpicture}[node distance=8mm, minimum size=12mm]
        % \footnotesize
        \node[state, initial] (q0) [] { $\scriptstyle \stateq_0/\textcolor{ETHGreen}{1}$ }; 
        \node[state] (q1) [above right = of q0, xshift=13mm, yshift=-3mm] { $\scriptstyle \stateq_1$ }; 
        \node[state, accepting] (q2) [below right = of q0, xshift=12mm, yshift=3mm] { $\scriptstyle \stateq_2/\textcolor{ETHRed}{0.3}$ }; 
        \draw[transition] (q0) edge[auto, bend left, sloped] node[minimum size=4mm]{ $\syma/{\scriptstyle 0.6}$ } (q1) 
        (q0) edge[auto, bend right, sloped] node[minimum size=4mm]{ $\symb/{\scriptstyle 0.4}$ } (q2)
        (q1) edge[auto, loop right] node[minimum size=4mm]{ $\symb/{\scriptstyle 0.1}$ } (q1)
        (q1) edge[auto] node[minimum size=4mm]{ $\syma/{\scriptstyle 0.9}$ } (q2)
        (q2) edge[auto, loop right] node[minimum size=4mm]{ $\symb/{\scriptstyle 0.7}$ } (q2) ;
    \end{tikzpicture}
    \begin{tabular}{ll}
            % $\pdens(\syma \mid \stateq_0)$ & 0.5 \\
            % $\pdens(\symb \mid \stateq_0)$ & 0.5 \\
            % $\pdens(\syma \mid \stateq_1)$ & 0.9 \\
            % $\pdens(\symb \mid \stateq_1)$ & 0.1 \\
            % $\pdens(\symb \mid \stateq_1)$ & 0.5 \\
            % $\pdens(\eos \mid \stateq_1)$ & 0.5 \\
            % \midrule \\
            % $\pdens(\syma)$ & $0$ \\
            \normalsize $\pdens(\syma \symb^n \syma \symb^m)\colon$ & \normalsize $\textcolor{ETHGreen}{1} \cdot 0.6 \cdot 0.1^n \cdot 0.9 \cdot 0.7^m \cdot \textcolor{ETHRed}{0.3}$ \\
            \normalsize $\pdens(\symb \symb^m)\colon$ & \normalsize $\textcolor{ETHGreen}{1} \cdot 0.4 \cdot 0.7^m \cdot \textcolor{ETHRed}{0.3}$
            % $\pdens(\symb)$ & $0.5 \cdot 0.5 = 0.25$ \\
            % $\pdens(\syma \symb)$ & $0.5 \cdot 0.9 \cdot 0.5 = 0.225$
    \end{tabular}  
    \caption{A weighted finite-state automaton defining a probability distribution over $\kleene{\set{\syma, \symb}}$.}
    \label{fig:example-fslm}
\end{figure}

% This allows us to define finite-state LMs as LMs specified by a PFSA.
\begin{definition}
    A language model $\pLM$ is \defn{finite-state} (an FSLM) if it can be represented by a PFSA, i.e., if there exists a PFSA $\automaton$ such that, for every $\str \in \kleene{\alphabet}$, $\pLM\left(\str\right) = \wfsa\left(\str\right)$.
\end{definition}
See \cref{fig:example-fslm} for an example of a PFSA defining an FSLM over $\alphabet = \set{\syma, \symb}$. 
Its support consists of the strings $\syma \symb^n \syma \symb^m$ and $\symb \symb^m$ for $n, m \in \Nzero$.\looseness=-1

An FSLM can be specified by multiple equivalent PFSAs in the sense that they all describe the same probability distribution.
The one with the smallest number of states is the minimal PFSA.
\begin{definition}
    Let $\pLM$ be an FSLN. 
    A PFSA $\wfsa$ is a \defn{minimal (deterministic) PFSA} for $\pLM$ if it defines the same probability distribution as $\pLM$ and there is no (deterministic) PFSA with fewer states defining the same probability distribution.
\end{definition}

==> sections/implications.tex <==
% \subsection{\hernnAcr{}s and Non-determinism}
\cref{lem:heaviside-rnns-regular,lemma:minsky-constr} formalize the equivalence between \hernnAcr{}s and deterministic PFSAs.
A direct corollary of this result is that \hernnAcr{}s are at most as expressive as deterministic PFSAs and, therefore, strictly less expressive as general, non-deterministic, PFSAs.\footnote{General PFSAs are, in turn, equivalent to probabilistic regular grammars and discrete Hidden Markov Models \citep{ICARD2020102308}.}
An example of a very simple non-deterministic PFSA, i.e., a PFSA whose distribution cannot be expressed by an \hernnAcr{} LM, is shown in \cref{fig:nondet-pfsa}.
\begin{figure}
    \centering
    % \footnotesize
    \begin{tikzpicture}[node distance = 15mm]
    \node[state, initial] (q0) [] { $\stateq_{0} / {1}$ }; 
    \node[state] (q1) [right = of q0, yshift=10mm] { $\stateq_{1}$ }; 
    \node[state] (q2) [right = of q0, yshift=-10mm] { $\stateq_{2}$ }; 
    \node[state, accepting] (q3) [right = of q1, yshift=-10mm] { $\stateq_{3} / {1}$ }; 
    \draw[transition] (q0) edge[bend left, above, sloped] node{ $\syma/{0.5}$ } (q1)
    (q0) edge[bend right, above, sloped] node{ $\syma/{0.5}$ } (q2)
    (q1) edge[above, loop above] node{ $\symb/{0.9}$ } (q1)
    (q2) edge[below, loop below] node{ $\symb/{0.1}$ } (q2)
    (q1) edge[bend left, above, sloped] node{ $\symc/{0.1}$ } (q3)
    (q2) edge[bend right, above, sloped] node{ $\symc/{0.9}$ } (q3) ;
    \end{tikzpicture}
    \caption{A non-determinizable PFSA. It assigns the string $\syma \symb^n \symc$ the probability $\wfsa\left(\syma \symb^n \symc\right) = 0.5 \cdot 0.9^n \cdot 0.1 + 0.5 \cdot 0.1^n \cdot 0.9$, which can not be expressed as a single term for arbitrary $n \in \Nzero$.}
    \label{fig:nondet-pfsa}
\end{figure}
Furthermore, even if a non-deterministic PFSA can be determinized, the number of states of the determinized machine can be exponential in the size of the non-deterministic one \citep{Buchsbaum1998}.
In this sense, non-deterministic PFSAs can be seen as exponentially compressed representations of finite-state LMs.
However, the compactness of this non-deterministic representation must be ``undone'' using determinization before it can be encoded by an \hernnAcr{}.
% This is a general limitation of the fact that RNNs are deterministic.

% The equivalence between \hernnAcr{} LMs and \dpfsaAcr{}s also allows us to establish a number of constraints on the probability distributions expressible by \hernnAcr{} LMs.
% For example, we know that the probability of any string under an \hernnAcr{} LM will be a rational number \citep{ICARD2020102308}.\footnote{However, note that not all probability distributions with rational probabilities can be defined by regular grammars.}
% As a special case, any distribution over a single-letter alphabet will also have a rational generating function \citep{ICARD2020102308}.

% Moreover, the connection of \hernnAcr{} LMs to \dpfsaAcr{}s allows us to draw on results from (weighted) formal language theory to manipulate and investigate \hernnAcr{} LMs.
% For example, we can apply general results on the tightness of language models based on \dpfsaAcr{}s to \hernnAcr{} LMs \citep{Du2023}.\footnote{Informally, the question of tightness concerns the question of whether the LM forms a valid probability distribution over $\kleene{\alphabet}$, which is not necessarily the case for locally normalized LMs such as RNN LMs.}
% Even if the \hernnAcr{} LM is not tight \textit{a priori}, the fact that the normalizing constant can be computed means that it can always be re-normalized to form a probability distribution over $\kleene{\alphabet}$.
% Furthermore, we can draw on the various results on the minimization of \dpfsaAcr{}s to reduce the size of the \hernnAcr{} implementing the LM.

While \cref{lem:heaviside-rnns-regular} focuses on \hernnAcr{} LMs and shows that they are finite-state, a similar argument could be made for any RNN whose activation functions map onto a finite set.
This is the case with any implementation of an RNN on a computer with finite-precision arithmetic---in that sense, all deployed RNNLMs are finite-state, albeit with a very large state space. 
In other words, one can view RNNs as very compact representations of large deterministic probabilistic finite-state automata whose transition functions are represented by the RNN's update function.
Furthermore, since the topology and the weights of the implicit \dpfsaAcr{} are determined by the RNN's update function, the \dpfsaAcr{} can be learned very flexibly yet efficiently based on the training data.
This is enabled by the sharing of parameters across the entire graph of the \dpfsaAcr{} instead of explicitly parametrizing every possible transition in the \dpfsaAcr{} or by hard-coding the allowed transitions as in \ngram{} LMs.


% \subsection{Probabilistic Regular Languages and Their Equivalence with \hernnAcr{} LMs}
% \Anej{
% \begin{itemize}
%     % \item They are equivalent to (deterministic?) discrete HMMs, and to regular grammars (deterministic?)
%     % \item We can use the algorithms and conditions from WFSAs to investigate RNNs, e.g., 
%     % \begin{itemize}
%     %     \item Conditions on tightness; Their pathsum can also always be computed (lem 11/12)
%     %     \item Minimization
%     % \end{itemize}
%     % \item Define any rational-valued finite-support probability distributions (thm 8, cor 9)
%     \item The probability of any string is a rational number
%     \item Over single-symbol alphabets, they define rational generating functions
% \end{itemize}
% }

% \cref{lem:heaviside-rnns-regular,lemma:minsky-constr} show that \hernnAcr{} LMs equivalent in expressive power to deterministic \dpfsaAcr{}s, which are less powerful than general PFSAs, 

% \subsection{\hernnAcr{}s as PFSAs}
% On the other hand, the fact that RNNs can only compactly represent a subset of finite-state LMs is also interesting.
% The language studied by \citet{hewitt-etal-2020-rnns} both can be very compactly represented by an \hernnAcr{} LM and has clear linguistic motivations.
% Investigating whether other linguistically-motivated phenomena in human language can be efficiently represented by \hernnAcr{} LMs seems like an interesting area of future work.

==> sections/minsky.tex <==
This section discusses the other direction of \cref{thm:elman-pfsa-euqivalent}, showing that a general \dpfsaAcr{} can be simulated by an \hernnAcr{} LM using a variant of the classic theorem originally due to \citet{Minsky1954}.
% Minsky, however, was only interested in unweighted automata.
We give the theorem a probabilistic twist, making it relevant to language modeling.
\begin{restatable}{reLemma}{minskyLemma} \label{lemma:minsky-constr}
Let $\wfsa = \wfsatuple$ be a \dpfsaAcr{}.
Then, there exists an \hernnAcr{} LM $\rnnlm$ with $\rnn$ of size $\nsymbols \nstates$ defining the LM $\pLM$ such that $\pLN\left(\str\right) = \wfsa\left(\str\right)$ for every $\str \in \kleene{\alphabet}$.\looseness=-1
\end{restatable}
% We describe the construction proving \cref{lemma:minsky-constr} in the next subsection.
We describe the full construction of an \hernnAcr{} LM simulating a given \dpfsaAcr{} in the next subsection.
The full construction is described to showcase the mechanism with which the \hernnAcr{} can simulate the transitions of a given FSA and give intuition on why this might, in general, require a large number of parameters in the \hernnAcr{}.
Many principles and constraints of the simulation are also reused in the discussion of the lower bounds on the size of the \hernnAcr{} required to simulate the \dpfsaAcr{}.

We first introduce a fact that makes it easier to talk about how an \hernnAcr{} can simulate a \dpfsaAcr{}.
We will be interested in conjoining elements of vectors in $\B^\hiddDim$, which can be performed by a \hernnAcr{} with appropriately set parameters.
\begin{fact} \label{fact:and}
    Let $\idxm \in \Zmod{\hiddDim}$, $\idxi_1, \ldots, \idxi_\idxm\in \Zmod{\hiddDim}$, and $\vx, \vv \in \B^\hiddDim$ with $\evv_{\idxi} = \ind{\idxi \in \set{\idxi_1, \ldots, \idxi_\idxm}}$.
    % \begin{equation}
    % \evv_{\idxi} = \ind{\idxi \in \set{\idxi_1, \ldots, \idxi_\idxm}}.
    % % \begin{cases}
    % %      1 & \textbf{if } \idxi \in \set{\idxi_1, \ldots, \idxi_\idxm} \\
    % %      0 & \otherwisecondition
    % % \end{cases}.
    % \end{equation}
    Then, $\heaviside\left(\vv^\top \vx - \left(\idxm - 1\right) \right) = 1$ if and only if $\evx_{\idxi_\idxk} = 1$ for all $\idxk = 1, \ldots, \idxm$.
    In other words, $\heaviside\left(\vv^\top \vx - \left(\idxm - 1\right) \right) = \evx_{\idxi_1} \wedge \cdots \wedge \evx_{\idxi_\idxm}$.
\end{fact}


% \begin{proof}[Proof of \cref{lemma:minsky-constr}]
\subsubsection{Weighted Minsky's Construction}

\begin{figure*}
    \centering
        \begin{tikzpicture}

            \node[align=center] (a1) {
                \begin{tikzpicture}[node distance = 8mm, minimum size = 5mm]
                    \footnotesize
                    \node[state, fill=ETHPurple!30, draw=ETHPurple!80] (q){ $\stateq$ }; 
                    \node[draw=none, fill=none] (q0) [left = of q] { }; 
                    \node[state] (q1) [above right = of q] { $\stateq'$ }; 
                    \node[state] (q2) [below right = of q] { $\stateq''$ }; 
                    \draw[transition] (q0) edge[ETHPurple, above, sloped] node{ $\syma/w_0$ } (q) 
                        (q) edge[above, sloped] node{ $\syma/w'$ } (q1) 
                        (q) edge[above, sloped] node{ $\symb/w''$ } (q2);
                \end{tikzpicture}
            };
            \node[align=center, below = of a1, yshift=1cm, fill=ETHPurple!10] (e1) { $\hiddState = \onehot{\stateq, \syma}$ };
            
            \node[align=center, right = of a1, xshift=8mm, yshift=18mm] (a2) {
                \begin{tikzpicture}[node distance = 8mm, minimum size = 5mm]
                    \footnotesize
                    \node[state] (q){ $\stateq$ }; 
                    \node[draw=none, fill=none] (q0) [left = of q] { }; 
                    \node[state, fill=ETHPetrol!20, draw=ETHPetrol!80] (q1) [above right = of q] { $\stateq'$ }; 
                    \node[state, fill=ETHPetrol!20, draw=ETHPetrol!80] (q2) [below right = of q] { $\stateq''$ }; 
                    \draw[transition] (q0) edge[above, sloped] node{ $\syma/w_0$ } (q) 
                        (q) edge[ETHPetrol, above, sloped] node{ $\syma/w'$ } (q1) 
                        (q) edge[ETHPetrol, above, sloped] node{ $\symb/w''$ } (q2);
                \end{tikzpicture}
            };
            \node[align=center, above = of a2, xshift=-1.3cm, yshift=-1.7cm, fill=ETHPetrol!10] (e2) { $\scriptstyle \recMtx \hiddState = \textcolor{ETHGreen}{\onehot{\stateq', \syma}} + \onehot{\stateq'', \symb}$ };
            
            \node[align=center, right = of a1, xshift=8mm, yshift=-18mm] (a3) {
                \begin{tikzpicture}[node distance = 8mm, minimum size = 5mm]
                    \footnotesize
                    \node[state, fill=ETHBronze!30, draw=ETHBronze!80] (q){ $\stateq$ }; 
                    \node[draw=none, fill=none] (q0) [left = of q] { }; 
                    \node[state, fill=ETHBronze!30, draw=ETHBronze!80] (q1) [above right = of q] { $\stateq'$ }; 
                    \node[state] (q2) [below right = of q] { $\stateq''$ }; 
                    \draw[transition] (q0) edge[ETHBronze, above, sloped] node{ $\syma/w_0$ } (q) 
                        (q) edge[ETHBronze, above, sloped] node{ $\syma/w'$ } (q1) 
                        (q) edge[above, sloped] node{ $\symb/w''$ } (q2);
                \end{tikzpicture} 
            };
            \node[align=center, below = of a3, xshift=-1.3cm, yshift=1.7cm, fill=ETHBronze!10] (e3) { $\scriptstyle \inMtx \onehot{\syma} = \onehot{\stateq, \syma} + \textcolor{ETHGreen}{\onehot{\stateq', \syma}}$ };

            \node[align=center, right = of a1, xshift=60mm] (a4) {
                \begin{tikzpicture}[node distance = 8mm, minimum size = 5mm]
                    \footnotesize
                    \node[state] (q4f){ $\stateq$ }; 
                    \node[draw=none, fill=none] (q40) [left = of q4f] { }; 
                    \node[state, fill=ETHGreen!30, draw=ETHGreen!80] (q41) [above right = of q4f] { $\stateq'$ }; 
                    \node[state] (q42) [below right = of q4f] { $\stateq''$ }; 
                    \draw[transition] (q40) edge[above, sloped] node{ $\syma/w_0$ } (q4f) 
                        (q4f) edge[ETHGreen, above, sloped] node(greenEdge){ $\syma/w'$ } (q41) 
                        (q4f) edge[above, sloped] node{ $\symb/w''$ } (q42);
                \end{tikzpicture}
            };
            
            % \node[align=center, below = of a4] (e4) { $\scriptstyle \heaviside\left(\recMtx \hiddState + \inMtx \onehot{\syma}\right) = \onehot{\stateq', \syma}$ };
            \node[align=center, below = of a4, yshift=1cm, fill=ETHGreen!10] (e4) { $\hiddState' = \textcolor{ETHGreen}{\onehot{\stateq', \syma}}$ };
            
            % \draw (a1) edge[auto, sloped] node[minimum size=4mm]{ $\recMtx \hiddStatet = \onehot{\stateq', \syma} + \onehot{\stateq'', \symb}$ } (a2)
            % (a1) edge[auto, sloped] node[minimum size=4mm]{ $\inMtx \onehot{\syma} = \onehot{\stateq, \syma} + \onehot{\stateq', \syma}$ } (a3) ;
            \draw[->] (a1) edge[above, sloped] node{\footnotesize Children} (a2)
            (a1) edge[above, sloped] node{\footnotesize $\syma$-reachable} (a3) 
            (a2) edge (a4) 
            (a3) edge (a4) ;
            % (a1) edge[auto, sloped] node[minimum size=4mm]{ $\heaviside\left(\recMtx \hiddStatet + \inMtx \onehot{\syma}\right) = \onehot{\stateq', \syma}$ } (a4);
            
            % \hiddStatet = \onehot{\stateq, \syma}
            
            % \recMtx \hiddStatet = \onehot{\stateq', \syma} + \onehot{\stateq'', \symb}
            
            % \inMtx \onehot{\syma} = \onehot{\stateq, \syma} + \onehot{\stateq', \syma}
            
            % \heaviside\left(\recMtx \hiddStatet + \inMtx \onehot{\syma}\right) = \onehot{\stateq', \syma}

            \node[align=center, above = of a4, xshift=10mm, yshift=-8mm, fill=ETHRed!10] (sm) {
                $\projfuncEosalphabetminus\left(\outMtx \hiddState'\right) = \begin{pmatrix}
                    \textcolor{ETHGreen}{\syma\colon w'} \\
                    \symb\colon w'' \\
                    \eos\colon 0
                \end{pmatrix}$
            }; 
            
            % \draw[->, ETHGreen] (a4.north) to[bend left] (sm.south);
            \draw[-Latex, ETHRed, out = 30, in = -15] (a4.east) to (sm.south);

        \end{tikzpicture}
        \caption{A high-level illustration of how the transition function of the FSA is simulated in Minsky's construction on a fragment of an FSA \textcolor{ETHPurple}{starting at $\stateq$} (encoded in $\hiddState$) and reading the symbol $\syma$. 
        The top path disjoins the representations of the \textcolor{ETHPetrol}{children} of $\stateq$, whereas the bottom path disjoins the representations of states \textcolor{ETHBronze}{reachable by} an $\syma$-transition. 
        The Heaviside activation \textcolor{ETHGreen}{conjoins} these two representations into $\hiddState'$ (rightmost fragment). 
        Projecting $\outMtx \hiddState'$ results in the vector defining the same probability distribution as the outcoming arcs of $\stateq$ (\textcolor{ETHRed}{red box}).}
        \label{fig:minsky-overview}
\end{figure*}

For a \dpfsaAcr{} $\wfsa = \wfsatuple$, we construct a \hernnAcr{} LM $\rnnlm$ with $\rnn = \elmanrnntuple$ defining the same distribution over $\kleene{\alphabet}$.
The idea is to simulate the transition function $\trans$ with the Elman update rule by appropriately setting $\recMtx$, $\inMtx$, and $\biasVech$.
The transition weights defining the stringsums are represented in $\outMtx$.

% \footnote{
% The formal definitions of the RNN parameters in this proof might not be intuitive on their own. 
% To help the reader understand the definitions, we provide a visual illustration of some of the components in \cref{app:minsky-vis}.}
Let $\ordering\colon \states \times \alphabet \rightarrow \Zmod{\nstates\nsymbols }$ be a bijection, i.e., an ordering of $\states \times \alphabet$, $\symordering\colon \alphabet \rightarrow \Zmod{|\alphabet|}$ an ordering of $\alphabet$, and $\eossymordering\colon \eosalphabet \rightarrow \Zmod{|\eosalphabet|}$ an ordering of $\eosalphabet$.
We use $\ordering$, $\symordering$, and $\eossymordering$ to define the one-hot encodings $\onehot{\cdot}$ of state-symbol pairs and of the symbols. 
That is, we assume that $\onehot{\stateq, \sym}_{\idxd} = \ind{\idxd = \ordering\left(\stateq, \sym\right)}$, and similar for $\onehot{\sym}$.

\paragraph{\hernnAcr{}'s hidden states.}
The hidden state $\hiddStatet$ of $\rnn$ will represent the one-hot encoding of the current state $\qt$ of $\wfsa$ at time $\tstep$ together with the symbol $\symt$ with which $\wfsa$ entered $\qt$.
Formally,
\begin{equation}
    % \qToHFun{\qt, \symt} \defeq \onehot{\left(\qt, \symt\right)} \in \B^{\nstates \nsymbols }.
    \hiddStatet = \onehot{\left(\qt, \symt\right)} \in \B^{\nstates \nsymbols }.
\end{equation}
There is a small caveat: How do we set the incoming symbol of $\wfsa$'s initial state $\qinit$?
As we show later, the symbol $\symt$ in $\hiddStatet = \onehot{\left(\qt, \symt\right)}$ does not affect the subsequent transitions---it is only needed to determine the target of the current transition. 
Therefore, we can set $\hiddStateZero = \onehot{\left(\qinit, \sym\right)}$ for any $\sym \in \alphabet$.
% \looseness=-1

\paragraph{Encoding the transition function.}
% First, we encode the transition function $\trans$.
The idea of defining $\recMtx$, $\inMtx$, and $\biasVech$ is for the Elman update rule to perform, upon reading $\symtplus$, element-wise conjunction between the representations of the children of $\qt$
% of all the states the $\wfsa$ can transition to from $\qt$ by reading \emph{any symbol} 
and the representation of the states $\wfsa$ can transition into after reading in $\symtplus$ from \emph{any state}.
The former is encoded in the recurrence matrix $\recMtx$, which has access to the current hidden state that encodes $\qt$ while the latter is encoded in the input matrix $\inMtx$, which has access to the one-hot representation of $\symtplus$.
Conjugating the entries in those two representations will, due to the determinism of $\wfsa$, result in a single non-zero entry: one representing the state which can be reached from $\qt$ (1\textsuperscript{st} component) using the symbol $\symtplus$ (2\textsuperscript{nd} component); see \cref{fig:minsky-overview}.

More formally, the recurrence matrix $\recMtx$ lives in $\B^{\nsymbols \nstates \times \nsymbols \nstates}$.
Each column $\recMtx_{\colon, \ordering\left(\stateq, \sym\right)}$ of the matrix represents the children of the state $\stateq$ in the sense that the column contains $1$'s at the indices corresponding to the state-symbol pairs $\left(\stateq', \sym'\right)$ such that $\wfsa$ transitions from $\stateq$ to $\stateq'$ after reading in the symbol $\sym'$.
That is, for $\stateq, \stateq' \in \states$ and $\sym, \sym' \in \alphabet$, we define
% \begin{equation}
%     \eRecMtx_{\ordering(\stateq', \sym'), \ordering(\stateq, \sym)} \defeq 
%     \begin{cases} 
%         1 &\mid \text{ if } \edge{\stateq}{\sym'}{\circ}{\stateq'} \in \trans \\ 
%         0 &\mid \text{ otherwise } \end{cases}.
% \end{equation}
\begin{equation} \label{eq:minsky-recmtx}
    \eRecMtx_{\ordering(\stateq', \sym'), \ordering(\stateq, \sym)} \defeq \ind{\edge{\qt}{\sym'}{\circ}{\stateq'} \in \trans}.
\end{equation}
Since $\sym$ is free, each column is repeated $\nsymbols$-times: once for every $\sym \in \alphabet$---this is why, after entering the next state, the symbol used to enter it does not matter anymore and, in the case of the initial state, any incoming symbol can be chosen to set $\hiddStateZero$.\looseness=-1

The input matrix $\inMtx$ lives in $\B^{\nsymbols \nstates \times \nsymbols }$ and encodes the information about which states can be reached by which symbols (from \emph{any} state).
The non-zero entries in the column corresponding to $\sym' \in \alphabet$ correspond to the state-symbol pairs $\left(\stateq', \sym'\right)$ such that $\stateq'$ is reachable with $\sym'$ from \emph{some} state:
% \begin{equation}
%     \eInMtx_{\ordering\left(\stateq', \sym'\right), \symordering\left(\sym'\right)} \defeq 
%     \begin{cases}
%         1 \mid \text{ if } \edge{\circ}{\sym'}{\circ}{\stateq'} \in \trans \\ 
%         0 \mid \text{ otherwise } 
%     \end{cases}.
% \end{equation}
\begin{equation}\label{eq:minsky-inmtx}
    \eInMtx_{\ordering\left(\stateq', \sym'\right), \symordering\left(\sym'\right)} \defeq \ind{\edge{\circ}{\sym'}{\circ}{\stateq'} \in \trans}.
\end{equation}
Lastly, we define the bias as $\biasVech \defeq -\one \in \R^{\nstates\nsymbols }$, which allows the Heaviside function to perform the needed conjunction.
The correctness of this process is proved in \cref{app:proofs} (\cref{lem:minsky-transitions}).

\paragraph{Encoding the transition probabilities.}
We now turn to the second part of the construction: Encoding the string acceptance weights given by $\wfsa$ into the probability distribution defined by $\rnn$.
We present two ways of doing that: Using the standard softmax formulation, where we make use of the extended real numbers, and with the sparsemax.\looseness=-1

The conditional probabilities assigned by $\rnn$ are controlled by the $|\eosalphabet| \times \nstates\nsymbols$-dimensional output matrix $\outMtx$.
Since $\hiddStatet$ is a one-hot encoding of the state-symbol pair $\qt, \symt$, the matrix-vector product $\outMtx \hiddStatet$ simply looks up the values in the $\ordering\left(\qt, \symt\right)^\text{th}$ column.
After being projected to $\SimplexEosalphabetminus$, the entry in the projected vector corresponding to some $\symtplus \in \eosalphabet$ should match the probability of that symbol given that $\wfsa$ is in the state $\qt$.
This is easy to achieve by simply encoding the weights of the outgoing transitions into the $\ordering\left(\qt, \symt\right)^\text{th}$ column, depending on the projection function used.
% Depending on the projection function used, the information about the transition weights has to be encoded differently.
This is especially simple in the case of the sparsemax formulation. 
By definition, in a PFSA, the weights of the outgoing transitions and the final weight of a state $\qt$ form a probability distribution over $\eosalphabet$ for every $\qt \in \states$.
Projecting those values to the probability simplex, therefore, leaves them intact.
We can therefore define
\begin{equation} \label{eq:minsky-outmtx}
\outMtx_{\eossymordering\left(\sym'\right) \ordering\left(\stateq, \sym\right)} \defeq 
\begin{cases} \transitionWeightFun{\edge{\stateq}{\sym'}{w}{\circ}} & \mid \textbf{if } \sym' \in \alphabet \\ 
\finalf\left(\stateq\right) & \mid \otherwisecondition \end{cases}.
\end{equation}
Projecting the resulting vector $\outMtx \hiddStatet$, therefore, results in a vector whose entries represent the transition probabilities of the symbols in $\eosalphabet$.

In the more standard softmax formulation, we proceed similarly but log the non-zero transition weights. 
Defining $\log{0} \defeq -\infty$, we set
\begin{equation} 
\outMtx_{\eossymordering\left(\sym'\right) \ordering\left(\stateq, \sym\right)} \defeq 
\begin{cases} \log{\transitionWeightFun{\edge{\stateq}{\sym'}{w}{\circ}}} & \mid \textbf{if } \sym' \in \alphabet \\ 
\log{\finalf\left(\stateq\right)} & \mid \otherwisecondition \end{cases}.
\end{equation}
It is easy to see that the entries of the vector $\softmaxfunc{\outMtx \hiddStatet}{}$ form the same probability distribution as the original outgoing transitions out of $\stateq$.
% This means that, if $\hiddStatet$ encodes the state-symbol pair $\left(\stateq, \sym\right)$, the vector $\outMtx \hiddStatet$ will copy the selected column in $\outMtx$ which contains the output weight for all out symbols $\sym'$ of $\stateq$, i.e., the entry $\outMtx \hiddState_{\symordering\left(\sym'\right)}$ contains the (log of the) weight on the arc $\edge{\stateq}{\sym'}{w}{\circ}$.
Over the course of an entire input string, these weights are multiplied as the RNN transitions between different hidden states corresponding to the transitions in the original \dpfsaAcr{} $\wfsa$.
The proof can be found in \cref{app:proofs} (\cref{lem:minsky-probs}).
This establishes the complete equivalence between \hernnAcr{} LMs and FSLMs.\footnote{The full discussion of the result is postponed to \cref{sec:discussion}.}

% \begin{figure*}
%     \centering
%         \begin{tikzpicture}
%           \matrix[matrix of math nodes, row sep=5mm] (mat) {
%             \begin{tikzpicture}[node distance = 8mm]
%             \footnotesize
%             \node[state, fill=ETHPurple!30, draw=ETHPurple!80] (q){ $\stateq$ }; 
%             \node[draw=none, fill=none] (q0) [left = of q, xshift=2mm] { }; 
%             \node[state] (q1) [above right = of q] { $\stateq'$ }; 
%             \node[state] (q2) [below right = of q] { $\stateq''$ }; 
%             \draw (q0) edge[ETHPurple, above, sloped] node{ $\syma/w_0$ } (q) 
%             (q) edge[above, sloped] node{ $\syma/w'$ } (q1) 
%             (q) edge[above, sloped] node{ $\symb/w''$ } (q2);
%             \end{tikzpicture}
%             &
%             \begin{tikzpicture}[node distance = 8mm]
%             \footnotesize
%             \node[state] (q){ $\stateq$ }; 
%             \node[draw=none, fill=none] (q0) [left = of q, xshift=2mm] { }; 
%             \node[state, fill=ETHPetrol!20] (q1) [above right = of q] { $\stateq'$ }; 
%             \node[state, fill=ETHPetrol!20] (q2) [below right = of q] { $\stateq''$ }; 
%             \draw (q0) edge[above, sloped] node{ $\syma/w_0$ } (q) 
%             (q) edge[ETHPetrol, above, sloped] node{ $\syma/w'$ } (q1) 
%             (q) edge[ETHPetrol, above, sloped] node{ $\symb/w''$ } (q2);
%             \end{tikzpicture} &
%             \begin{tikzpicture}[node distance = 8mm]
%             \footnotesize
%             \node[state, fill=ETHBronze!30, draw=ETHBronze!80] (q){ $\stateq$ }; 
%             \node[draw=none, fill=none] (q0) [left = of q, xshift=2mm] { }; 
%             \node[state, fill=ETHBronze!30, draw=ETHBronze!80] (q1) [above right = of q] { $\stateq'$ }; 
%             \node[state] (q2) [below right = of q] { $\stateq''$ }; 
%             \draw (q0) edge[ETHBronze, above, sloped] node{ $\syma/w_0$ } (q) 
%             (q) edge[ETHBronze, above, sloped] node{ $\syma/w'$ } (q1) 
%             (q) edge[above, sloped] node{ $\symb/w''$ } (q2);
%             \end{tikzpicture} 
%             \begin{tikzpicture}[node distance = 8mm]
%             \footnotesize
%             \node[state] (q){ $\stateq$ }; 
%             \node[draw=none, fill=none] (q0) [left = of q, xshift=2mm] { }; 
%             \node[state, fill=ETHGreen!30, draw=ETHGreen!80] (q1) [above right = of q] { $\stateq'$ }; 
%             \node[state] (q2) [below right = of q] { $\stateq''$ }; 
%             \draw (q0) edge[ETHGreen, above, sloped] node{ $\syma/w_0$ } (q) 
%             (q) edge[above, sloped] node{ $\syma/w'$ } (q1) 
%             (q) edge[above, sloped] node{ $\symb/w''$ } (q2);
%             \end{tikzpicture} \\
%             \hiddStatet = \onehot{\stateq, \syma}
%             &
%             \recMtx \hiddStatet = \onehot{\stateq', \syma} + \onehot{\stateq'', \symb}
%             &
%             \inMtx \onehot{\syma} = \onehot{\stateq, \syma} + \onehot{\stateq', \syma}
%             &
%             \heaviside\left(\recMtx \hiddStatet + \inMtx \onehot{\syma}\right) = \onehot{\stateq', \syma}\\
%           };
%         \end{tikzpicture}
%         \caption{A high-level illustration of how the transition function of the FSA is implemented in Minsky's construction.}
%         \label{fig:minsky-overview}
% \end{figure*}



==> sections/proofs.tex <==
\hernnRegularLemma*
\begin{proof}%[Proof of \cref{lem:heaviside-rnns-regular}]
Let $\rnn = \elmanrnntuple$ be a \hernnAcr{} defining the conditional probabilities $\pLNSM$.
We construct a deterministic PFSA $\wfsa = \wfsatuple$ defining the same string probabilities.
% \anej{I avoided specifying sequence/language models here as it is not central. However, this proof of course works for non-tight models as well. Do we include non-tight models?}
Let $\hToQ\colon \B^\hiddDim \to \Z_{2^\hiddDim}$ be a bijection.
Now, for every state $\stateq \defeq \hToQFun{\vh} \in \states \defeq \B^\hiddDim$, construct a transition $\edge{\stateq}{\sym}{w}{\stateq'}$ where $\stateq' = \elmanUpdate{\vh}{\sym}$ with the weight $w = \pLNSM\left(\sym \mid \vh\right) = \projfuncEosalphabetminusFunc{\outMtx \, \vh}_{\sym}$.
We define the initial function as $\initf\left(\hToQFun{\vh}\right) = \ind{\vh = \hiddStateZero}$ and final function $\finalf$ with $\finalf\left(\stateq\right) \defeq \pLNSM\left(\eos \mid \hToQFun{\stateq}\right)$.

It is easy to see that $\wfsa$ defined this way is deterministic.
We now prove that the weights assigned to strings by $\wfsa$ and $\rnn$ are the same.
Let $\str \in \kleene{\alphabet}$ with $|\str| = \strlen$ and 
\[
    \apath = \left(\edge{\hToQFun{\hiddStateZero}}{\sym_1}{w_1}{\stateq_1}, \ldots, \edge{\qT}{\sym_{\strlen}}{w_{\strlen}}{\stateq_{\strlen + 1}}\right)
\]
the $\str$-labeled path starting in $\hToQFun{\hiddStateZero}$ (such a path exists since we the defined automaton is \emph{complete}---all possible transitions are defined for all states).
\begin{align*}
    \wfsa\left(\str\right) =& \initf\left(\hToQFun{\hiddStateZero}\right) \cdot \left[\prod_{\tstep = 1}^{\strlen} w_\tstep\right] \cdot \finalf\left(\stateq_{\strlen + 1}\right) \\
    =& 1 \cdot \prod_{\tstep = 1}^{\strlen}\pLNSM\left(\symt \mid \hToQinvFun{\stateq_\tstep}\right) \cdot \pLNSM\left(\eos \mid \hToQinvFun{\stateq_{\strlen + 1}}\right) \\
    =& \pLN\left(\str\right)
\end{align*}
which is exactly the weight assigned to $\str$ by $\rnn$.
Note that all paths not starting in $\hToQFun{\hiddStateZero}$ have weight $0$ due to the definition of the initial function.
\end{proof}

\begin{lemma} \label{lem:minsky-transitions}
    Let $\wfsa = \wfsatuple$ be a deterministic PFSA, $\str = \sym_1\ldots\sym_\strlen \in \kleene{\alphabet}$, and $\qt$ the state arrived at by $\wfsa$ upon reading the prefix $\strlet$.
    Let $\rnn$ be the \hernnAcr{} specified by the Minsky construction for $\wfsa$, $\ordering$ the ordering defining the one-hot representations of state-symbol pairs by $\rnn$, and $\hiddStatet$ $\rnn$'s hidden state after reading $\strlet$.
    Then, it holds that $\hiddStateZero = \onehot{\left(\qinit, \sym\right)}$ where $\qinit$ is the initial state of $\wfsa$ and $\sym \in \alphabet$ and $\hiddStateT = \onehot{\left(\qT, \sym_\strlen\right)}$.
\end{lemma}
\begin{proof}
Define $\hToQFun{\hiddState = \onehot{\left(\stateq, \sym\right)}} \defeq \stateq$.
We can then restate the lemma as $\hToQFun{\hiddStateT} = \qT$ for all $\str \in \kleene{\alphabet}$, $|\str| = \strlen$.
% Let $\str \in \kleene{\alphabet}$ with $|\str| = \strlen$.
Let $\apath$ be the $\str$-labeled path in $\wfsa$.
We prove the lemma by induction on the string length $\strlen$.
\paragraph{Base case: $\strlen = 0$.}
Holds by the construction of $\hiddStateZero$.
\paragraph{Inductive step: $\strlen > 0$.}
Let $\str \in \kleene{\alphabet}$ with $|\str| = \strlen$ and assume that $\hToQFun{\hiddState_{\strlen - 1}} = \stateq_{\strlen - 1}$.

We prove that the specifications of $\recMtx$, $\inMtx$, and $\biasVech$ ensure that $\hToQFun{\hiddStateT} = \qT$. 
By definition of the recurrence matrix $\recMtx$ (cf. \cref{eq:minsky-recmtx}), the vector $\recMtx \hiddStateTminus$ will contain a $1$ at the entries $\ordering\left(\stateq', \sym'\right)$ for $\stateq' \in \states$ and $\sym' \in \alphabet$ such that $\edge{\qTminus}{\sym'}{\circ}{\stateq'} \in \trans$.
This can equivalently be written as $\recMtx \hiddStateTminus = \bigvee_{\edge{\qTminus}{\sym'}{\circ}{\stateq'} \in \trans} \onehot{\left(\stateq', \sym'\right)}$, where the disjunction is applied element-wise.

On the other hand, by definition of the input matrix $\inMtx$ (cf. \cref{eq:minsky-inmtx}), the vector $\inMtx \onehot{\symT}$ will contain a $1$ at the entries $\ordering\left(\stateq', \symT\right)$ for $\stateq' \in \states$ such that $\edge{\circ}{\symT}{\circ}{\stateq'} \in \trans$.
This can also be written as $\inMtx \onehot{\symT} = \bigvee_{\edge{\circ}{\symT}{\circ}{\stateq'} \in \trans} \onehot{\left(\stateq', \symT\right)}$.

By \cref{fact:and}, $\heaviside\left(\recMtx \hiddStateTminus + \inMtx \onehot{\symT} + \biasVech\right)_{\ordering\left(\stateq', \sym'\right)} = \heaviside\left(\recMtx \hiddStateTminus + \inMtx \onehot{\symT} - \one \right)_{\ordering\left(\stateq', \sym'\right)} = 1$ holds if and only if $\left(\recMtx \hiddStateTminus\right)_{\ordering\left(\stateq', \sym'\right)} = 1$ and $\left(\inMtx \onehot{\symT}\right)_{\ordering\left(\stateq', \sym'\right)} = 1$.
This happens if 
\begin{equation}
    \edge{\qTminus}{\sym'}{\circ}{\stateq'} \in \trans \text{ and } \edge{\circ}{\symT}{\circ}{\stateq'} \in \trans \iff \edge{\qTminus}{\symT}{\circ}{\stateq'},
\end{equation}
i.e., if and only if $\wfsa$ transitions from $\qTminus$ to $\qT$ upon reading $\symT$ (it transitions only to $\qT$ due to determinism).

Since the string $\str$ was arbitrary, this finishes the proof.
\end{proof}

\begin{lemma}\label{lem:minsky-probs}
    Let $\wfsa = \wfsatuple$ be a deterministic PFSA, $\str = \sym_1\ldots\sym_\strlen \in \kleene{\alphabet}$, and $\qt$ the state arrived at by $\wfsa$ upon reading the prefix $\strlet$.
    Let $\rnn$ be the \hernnAcr{} specified by the Minsky construction for $\wfsa$, $\outMtx$ the output matrix specified by the generalized Minsky construction, $\ordering$ the ordering defining the one-hot representations of state-symbol pairs by $\rnn$, and $\hiddStatet$ $\rnn$'s hidden state after reading $\strlet$.
    Then, it holds that $\pLN\left(\str\right) = \wfsa\left(\str\right)$.    
\end{lemma}
\begin{proof}
% We now prove that the \hernnAcr{} $\rnn$ assigns strings $\str \in \kleene{\alphabet}$ the same probabilities as $\wfsa$.
Let $\str \in \kleene{\alphabet}$, $|\str| = \strlen$ and let $\apath$ be the $\str$-labeled path in $\wfsa$.
Again, let $\overline{\pdens}\left(\str\right) \defeq \prod_{\tstep = 1}^{|\str|} \pLNSMFun{\symt}{\strlt}$.
% is the state arrived at by $\wfsa$ after reading in $\str$.
We prove $\overline{\pdens}\left(\str\right) = \prod_{\tstep = 1}^\strlen w_\tstep$ by induction on $\strlen$.
\paragraph{Base case: $\strlen = 0$.}
In this case, $\str = \eps$, i.e., the empty string, and $\wfsa\left(\eps\right) = 1$.
$\rnn$ computes $\overline{\pdens}\left(\eps\right) = \prod_{\tstep =1 }^{0} \pLNSM\left(\symt\mid\strlt\right) = 1$. 
\paragraph{Inductive step: $\strlen > 0$.}
% Suppose that the $\overline{\pdens}\left(\str\right) = \prod_{\tstep = 1}^{\strlen'} w_\tstep$ for all $\strlen' < \strlen$.
Assume that the $\overline{\pdens}\left(\sym_1 \ldots \symTminus\right) = \prod_{\tstep = 1}^{\strlen - 1} w_\tstep$.
By \cref{lem:minsky-transitions}, we know that $\hToQFun{\hiddStateTminus} = \qTminus$ and $\hToQFun{\hiddStateT} = \qT$.
% Let $\str_{<\strlen} \in \kleene{\alphabet}$ and $\str_{\leq \strlen} \defeq \str_{<\strlen} \sym$ for some $\sym \in \alphabet$.
% Then, $\overline{\pdens}\left(\strlt\right) = \prod_{\tstep = 1}^{\strlen - 1} w_\tstep$ and, again, we know that $\hToQFun{\hiddState_{\strlen-1}} = \qT$ and $\hToQFun{\hiddStateT} = \stateq_{\strlen + 1}$, i.e.,  the states arrived at by $\wfsa$ after reading $\strlt$ and $\str_{\leq \strlen}$, respectively. 
By the definition of $\outMtx$ for the specific $\projfuncEosalphabetminus$, it holds that $\projfuncEosalphabetminusFunc{\outMtx \hiddState_{\strlen - 1}}_{\symordering\left(\sym\right)} = \transitionWeightFun{\edge{\hToQFun{\hiddState_{\strlen-1}}}{\sym}{w_\strlen}{\hToQFun{\hiddState_{\strlen}}}} = w_\strlen$.
This means that $\overline{\pdens}\left(\str_{\leq \strlen}\right) = \prod_{\tstep = 1}^{\strlen} w_\tstep$, which is what we wanted to prove.

Clearly, $\pLN\left(\str\right) = \overline{\pdens}\left(\str\right) \pLNSM\left(\eos \mid \str\right)$.
By the definition of $\outMtx$ (cf. \cref{eq:minsky-outmtx}), $\left(\outMtx \hiddStateT\right)_{\symordering\left(\eos\right)} = \finalf\left(\hToQFun{\hiddStateT}\right)$, meaning that $\pLN\left(\str\right) = \overline{\pdens}\left(\str\right) \pLNSM\left(\eos \mid \str\right) = \prod_{\tstep = 1}^{\strlen} w_\tstep\finalf\left(\hToQFun{\hiddStateT}\right) = \wfsa\left(\str\right)$.
Since $\str \in \kleene{\alphabet}$ was arbitrary, this finishes the proof.
% This means that, as long as $\overline{\pdens}\left(\str\right) = \prod_{\tstep = 1}^\strlen w_\tstep$, where $w_\tstep$ are the weights of the $\str$-labeled path in $\wfsa$, $\pLN\left(\str\right) = \wfsa\left(\str\right)$ holds.

% Let $\stateq$ be the state arrived at by $\wfsa$ after reading in the string $\str \in \kleene{\alphabet}$.
% The RNN $\rnn$ computes the probability $\pLNSM\left(\sym\mid\str\right)$ as 
% \begin{align} \label{eq:rnn-minsky-locally-correct}
%     &\pLNSM\left(\sym\mid\str\right) = \softmaxfunc{\outMtx \qToHFun{\stateq}}{\sym} \\
%     &= \begin{cases}  \displaystyle
%         \frac{\exp\left[\log w\right]}{\underset{ \scriptscriptstyle  \edge{\stateq}{\sym'}{w'}{\stateq'}}{\mathlarger{\sum}} \exp\left[\log w'\right] + \exp\left[\log \finalf\left(\stateq\right)\right]} & \textbf{if } \edge{\circ}{\sym}{w}{\circ} \in \trans \\
%         0 & \textbf{otherwise}
%     \end{cases} \\
%     &= \begin{cases} \displaystyle
%         \frac{w}{\underset{ \scriptscriptstyle \edge{\stateq}{\sym'}{w'}{\stateq'} }{\mathlarger{\sum}}w' + \finalf\left(\stateq\right)} = w & \textbf{if } \edge{\circ}{\sym}{w}{\circ} \in \trans \\
%         0 & \textbf{otherwise}
%     \end{cases}
% \end{align}
% The last step used the fact that $\wfsa$ is locally normalized, meaning that the denominator is $1$.
% Similarly, it holds that
% \begin{equation}
%     \pLNSM\left(\eos\mid\str\right) = \finalf\left(\stateq\right),
% \end{equation}
% where $\stateq$ is the state arrived at by $\wfsa$ after reading in $\str$.

% To show that the RNN $\rnn$ indeed encodes the same weighted language as $\wfsa$, we consider its locally normalized model.
% Clearly, the $-\infty$ logits in the conditionals $\pLNSM\left(\sym\mid \str\right)$ zero out the probability of any string not in the support of $\wfsa$.
% Suppose now that $\str \in \kleene{\alphabet}$ such that $\wfsa\left(\str\right) \neq 0$. 
% Let $\apath = \left(\edge{\qinit}{\sym_1}{w_1}{\stateq_1}, \ldots, \edge{\stateq_{\strlen - 1}}{\sym_{\strlen}}{w_{\strlen}}{\stateq_{\strlen}}\right)$ be the the $\str$-labeled path where $\qinit$ is the sole initial state of $\wfsa$.
% The RNN $\rnn$ computes the probability $\pLN\left(\str\right)$ with $\strlen = |\str|$ as
% \begin{align*}
%     \pLN\left(\str\right) &= \pLNSM\left(\eos\mid \str\right) \prod_{\tstep = 1}^{\strlen} \pLNSM\left(\sym\mid \str\right) \\
%     &= \finalf\left(\qT\right) \prod_{\tstep = 1}^{\strlen} w_\tstep
%     = \wfsa\left(\str\right)
% \end{align*}
% where we took into account that $\wfsa$ is deterministic and therefore only has one initial state with the initial weight $1$.
% This finishes the proof of the lemma.

\end{proof}


\statesLowerBound*
\begin{proof}
Without loss of generality, we work with $\Rex$-valued hidden states.
Let $\wfsa$ be a minimal deterministic PFSA and $\rnn = \elmanrnntuple$ a \hernnAcr{} with $\pLN\left(\str\right) = \wfsa\left(\str\right)$ for every $\str \in \kleene{\alphabet}$.
Let $\str_{<\strlen} \in \kleene{\alphabet}$ and $\str_{\leq \strlen} \defeq \str_{<\strlen} \sym$ for some $\sym \in \alphabet$.
Define $\overline{\pdens}\left(\str\right) \defeq \prod_{\tstep = 1}^{|\str|} \pLNSMFun{\symt}{\strlt}$.
It is easy to see that $\overline{\pdens}\left(\str_{<\strlen} \sym_\strlen\right) = \overline{\pdens}\left(\str_{<\strlen}\right)\pLNSMFun{\symt}{\str_{<\strlen}}$.
The conditional distribution $\pLNSM\left(\cdot \mid \str_{<\strlen}\right)$ are proportional to the values in $\outMtx \hiddState_{\strlen - 1}$.
By definition of the deterministic PFSA, there are $\nstates$ such conditional distributions.
Moreover, these distributions (represented by vectors $\in \SimplexEosalphabetminus$) can generally be \emph{linearly independent}.
This means that for any $\stateq$, the probability distribution of the outgoing transitions can not be expressed as a linear combination of the probability distributions of other states.
To express the probability vectors for all states, the columns of the output matrix $\outMtx$, therefore, have to span $\Rex^{\nstates}$, implying that $\outMtx$ must have at least $\nstates$ columns.
This means that the total space complexity (and thus the size of the \hernnAcr{} representing the same distribution as $\wfsa$) is $\Omega\left(\nstates\right)$.
\end{proof} 

==> sections/rnns.tex <==
\defn{RNN LMs} are LMs whose conditional distributions are given by a recurrent neural network.
Over the course of this paper, we will focus on Elman RNNs \citep{Elman1990} as they are the easiest to analyze and special cases of more common networks, e.g., those based on long short-term memory \citep[LSTM;][]{10.1162/neco.1997.9.8.1735} and gated recurrent units \citep[GRUs;][]{cho-etal-2014-properties}.\looseness=-1
% Formally, an Elman network is an RNN as follows.
\begin{definition} \label{def:elman-rnn}
% Let $\alphabet$ be an alphabet.
% , $\eos$ be a distinguished token \emph{not} in $\alphabet$, and $\eosalphabet = \alphabet \cup \{\eos\}$ be the $\eos$-augmented alphabet.
An \defn{Elman RNN} (\ernnAcr{}) $\rnn = \elmanrnntuple$ is an RNN with the following hidden state update rule: 
\begin{equation} \label{eq:elman-update-rule}
\hiddStatet \defeq \sigmoid\left(\recMtx \vhtminus + \inMtx \inEmbedSymt + \biasVech \right),
\end{equation}
where $\hiddStateZero$ is set to some vector in $\R^\hiddDim$.
$\inEmbedding\colon \eosalphabet \to \R^\embedDim$ is the symbol representation function 
% which represents each symbol $\sym \in \alphabet$ as a $\embedDim$-dimensional vector 
and $\sigmoid$ is an element-wise nonlinearity.
$\biasVech \in \R^{\hiddDim}$, $\recMtx \in \R^{\hiddDim \times \hiddDim}$, and $\inMtx \in \R^{\hiddDim \times \embedDim}$. 
We refer to the dimensionality of the hidden state, $\hiddDim$, as the \defn{size} of the RNN.
% $\embedDim$ is the dimensionality of the symbol representations $\inEmbedSym$.\anej{do we really need e'?}
\end{definition}

An RNN $\rnn$ specifies an LM by 
% the probability of a string $\str \in \kleene{\alphabet}$ as
% \begin{equation}
%     \pLN(\str) \defeq \pLNSM(\eos \mid \str) \prod_{\tstep=1}^\strlen \pLNSM(\symt \mid \str_{<\tstep}) 
% \end{equation}
% where we define the
% defining the conditional distributions for $\symt$ given $\strlt$ with the softmax function as
defining the conditional distributions for $\symt$ given $\strlt$.
\begin{definition}
    Let $\outMtx \in \R^{|\eosalphabet| \times \hiddDim}$ and let $\rnn$ be an RNN.
    An \defn{RNN LM} $\rnnlm$ is an LM whose conditional distributions are defined by 
    % linearly transforming $\hiddStatet$ with $\outMtx$ and projecting the 
    projecting $\outMtx \hiddStatet$ onto the probability simplex $\SimplexEosalphabetminus$ using some $\projfuncEosalphabetminus\colon \Rhid \to \SimplexEosalphabetminus$:
    \begin{equation}
    \pLNSM(\symt \mid \str_{<\tstep}) \defeq \projfuncEosalphabetminusFunc{\outMtx \hiddStatet}_{\symt}.
    \end{equation}
    We term $\outMtx$ the \defn{output matrix}.
\end{definition}
% In an RNNLM, the RNN intuitively provides the representation of the \defn{context} $\strlt$ which is transformed into the logits of the conditional distribution using the output matrix.
% $\outMtx$ is the \defn{output matrix}.

The most common choice for $\projfuncEosalphabetminus$ is the \defn{softmax} defined for $\vx \in \Rhid$ and $\idxd \in \Zmod{\hiddDim}$ as\looseness=-1
\begin{equation}
    \softmaxfunc{\vx}{\idxd} \defeq \frac{\exp\left[\evx_\idxd\right]}{\sum_{\idxd' = 1}^{\hiddDim} \exp{\left[\evx_{\idxd'}\right]}}.
\end{equation}
An important limitation of the softmax is that it results in a distribution with full support for all $\vx \in \Rhid$.
However, one can achieve $0$ probabilities by including \emph{extended} real numbers $\Rex \defeq \R \cup \set{-\infty, \infty}$: Any element with $\evx_\idxd = -\infty$ will result in $\softmaxfunc{\vx}{\idxd} = 0$.
% We will use this in our constructions below.

Recently, a number of alternatives to the softmax have been proposed.
This paper uses the sparsemax function \citep{sparsemax}, which can output sparse distributions:\looseness=-1
\begin{equation}\label{eq:spmax}
    \sparsemaxfunc{\vx}{} \defeq \argmin_{\rvp\in \Simplexdminus} ||\rvp- \vx ||^2_2.
\end{equation}
% Intuitively, the projection of $\vx \in \Rhid$ is likely to fall on the boundary of the probability simplex, resulting in a sparse categorical distribution.
Importantly, $\sparsemaxfunc{\vx}{} = \vx$ for $\vx \in \Simplexdminus$.
% \begin{align}
% \pLNSM(\symt \mid \str_{<\tstep}) &\defeq \softmaxfunc{\outMtx \hiddStatet}{\symt} \\
% &\defeq \frac{\exp\left[\inner{\embedSymt}{\hiddStatet}\right]}{\sum_{\sym' \in \eosalphabet} \exp{\left[\inner{\embedSymPrime}{\hiddStatet}\right]}}.
% \end{align}
% $\outMtx \in \R^{|\eosalphabet| \times \hiddDim}$ is the \defn{output matrix} used to define the logits of the conditional distributions.
% The RNN, therefore, intuitively provides the representation of the \defn{context} $\strlt$ which is transformed into the logits of the conditional distribution using the output matrix.

\paragraph{On determinism.}
Unlike WFSAs, Elman RNNs (and most other popular RNN architectures, such as the LSTM and GRU) are inherently deterministic.
% This is especially important since not all non-deterministic WFSAs admit an equivalent deterministic machine.
As we show shortly, certain types of Elman RNNs are at most as powerful as deterministic WFSAs, meaning that they can not represent non-determinizable WFSAs.
% ---this makes RNNs strictly less powerful than general WFSAs.

% \paragraph{Hard Thresholding}
Common choices for the nonlinear function $\sigmoid$ in \cref{eq:elman-update-rule} are the sigmoid function $\sigmoid(x) = \frac{1}{1 + \exp\left[x\right]}$ and the ReLU $\sigmoid(x) = \max(0, x)$. 
However, the resulting nonlinear interactions of the parameters and the inputs make the analysis of RNN LMs challenging.
One fruitful manner to make the analysis tractable is making simplifying assumptions on $\sigmoid$.
A common simplification is the use of the Heaviside activation function \citep{McCulloch1943,Minsky1954,Kleene1956,Dewdney1977,Alon1991EfficientSO,Indyk95}.
\begin{definition} \label{def:heaviside}
The \defn{Heaviside} function is defined as $\heaviside(x) \defeq \ind{x > 0}$.
\end{definition}
% In words, the Heaviside function maps every real value either $0$ or $1$, depending on whether it is greater than or less than zero. 
We will refer to the set $\set{0, 1}$ as $\B \defeq \set{0, 1}$.

With this, we can define the Heaviside \ernnAcr{}, the main object of study in the rest of the paper.
% A thresholding Elman network is an Elman recurrent neural network with the thresholding sigmoid.
\begin{definition}
A \defn{Heaviside Elman network} (\hernnAcr{}) is an \ernnAcr{} with Heaviside function $\heaviside$ as the nonlinearity $\sigmoid$.
\end{definition}


==> sections/space-bounds.tex <==
\cref{lemma:minsky-constr} shows that \hernnAcr{} LMs are at least as powerful as \dpfsaAcr{}s. 
More precisely, it shows that any \dpfsaAcr{} $\wfsa = \wfsatuple$ can be simulated by an \hernnAcr{} LM of size $\bigO{\nstates \nsymbols}$.
In this section, we address the following question: How large does an \hernnAcr{} LM have to be such that it can correctly simulate a \dpfsaAcr{}?
We study the asymptotic bounds with respect to the size of the set of states, $\nstates$, as well as the number of symbols, $\nsymbols$.

\subsection{Asymptotic Bounds in $\nstates$}
Intuitively, the $2^\hiddDim$ configurations of a $\hiddDim$-dimensional \hernnAcr{} hidden state could represent $2^\hiddDim$ states of a (dP)FSA.
One could therefore expect that we could achieve exponential compression of a \dpfsaAcr{} by representing it as an \hernnAcr{} LM.
Interestingly, this is not possible in general: Extending work by \citet{Dewdney1977}, \citet{Indyk95} shows that, to represent an unweighted FSA with an \hernnAcr{}, one requires an \hernnAcr{} of size $\Omega\left(\nsymbols \sqrt{\nstates}\right)$.
This lower bound can be achieved.\footnote{For completeness, we present constructions by \citet{Dewdney1977} and \citet{Indyk95}, which represent an unweighted FSA with a \hernnAcr{} of size $\bigO{\nsymbols\nstates^{\frac{3}{4}}}$ and $\bigO{\nsymbols\sqrt{\nstates}}$, respectively, in \cref{sec:dewdney-indyk}.}

% Since the lower bound of $\Omega\left(\nsymbols\sqrt{\nstates}\right)$ from the unweighted case generalizes to the weighted one, w
We now ask whether the same lower bound can also be achieved when simulating \dpfsaAcr{}s.
We find that the answer is negative: \dpfsaAcr{}s may require an \hernnAcr{} LMs of size $\Omega\left(\nsymbols\nstates\right)$ to faithfully represent their probability distribution.
% More precisely, the transition function can still be simulated in an ``unweighted'' fashion as shown in the generalized Minsky's construction.
Since the transition function of the underlying FSA can be simulated with more efficient constructions, the bottleneck comes from defining the same probability distribution.
Indeed, as the proof of the following theorem shows (\cref{thm:pfsa-rnn-lower-bound} in \cref{app:proofs}), the issue intuitively arises in the fact that, unlike in an \hernnAcr{} LM, the local probability distributions of the different states in a PFSA are completely arbitrary, whereas they are defined by shared parameters (the output matrix $\outMtx$) in an \hernnAcr{} LM.
\begin{restatable}{reTheorem}{statesLowerBound} \label{thm:pfsa-rnn-lower-bound}
Let $\wfsa = \wfsatuple$ be a minimal \dpfsaAcr{} and $\rnnlm$ an \hernnAcr{} LM defining the same LM. 
Then, $\hiddDim$ must scale linearly with $\nstates$.
% Then $\hiddDim = \Omega\left(\nsymbols \nstates\right)$.
\end{restatable}
% \cref{thm:pfsa-rnn-lower-bound} establishes a lower bound on the size of \hernnAcr{}s simulating arbitrary \dpfsaAcr{}s.
% This does not mean that no PFSAs can be simulated efficiently by \hernnAcr{}s.
Note that there exist regular languages motivated by phenomena in human language that \emph{can} be represented in logarithmic space in the number of the states of their minimal FSA.
For example, \citet{hewitt-etal-2020-rnns} show that bounded Dyck languages of $k$ parenthesis types and of maximal depth $m$, which require an FSA with $k^m$ states to be recognized, can be represented by \hernnAcr{} LMs of size $m \log{k}$, which is an exponential improvement on Indyk's lower bound. \looseness=-1

\subsection{Asymptotic Bounds in $\nsymbols$}
% We now characterize lower bounds in the size of the \hernnAcr{} LM with respect to the size of the PFSA alphabet, $\nsymbols$.
Since each of the input symbols can be encoded in $\log \nsymbols$ bits, one could expect that the linear factor in the size of the alphabet from the constructions above could be reduced to $\bigO{\log\nsymbols}$. 
However, we again find that such reduction is in general not possible---the set of FSAs presented in \cref{sec:alphabet-bounds} is an example of a family that requires an \hernnAcr{} whose size scales linearly with $\nsymbols$ to be simulated correctly, which implies the following theorem.
\begin{restatable}{reTheorem}{symbolsLowerBound} \label{thm:pfsa-rnn-lower-bound-alphabet}
Let $\wfsa = \wfsatuple$ be a minimal \dpfsaAcr{} and $\rnnlm$ an \hernnAcr{} LM defining the same LM. 
Then, $\hiddDim$ must scale linearly with $\nsymbols$.
\end{restatable}

% The main challenge in compressing the input symbols in the previous example was that there were many symbols leading to the same next state, whose representations were disjoined into a fully-active vector of all ones.
Based on the challenges encountered in the example from \cref{sec:alphabet-bounds}, we devise a simple sufficient condition for a logarithmic compression w.r.t. $\nsymbols$ to be possible: Namely, that for any pair of states $\stateq, \stateq' \in \states$, there is at most a single transition leading from $\stateq$ to $\stateq'$.
% is to require a simple structure on the nature of the transition function---namely, that there is at most 
Importantly, this condition is met by classical \ngram{} LMs, and also in the language studied by \citet{hewitt-etal-2020-rnns}, which allowed them to reduce the complexity w.r.t. $\nsymbols$ to the logarithmic factor.
This intuitive characterization can be formalized by a property we call $\log\nsymbols$-separability.
\begin{definition}
    An FSA $\wfsa = \fsatuple$ is \defn{$\log\nsymbols$-separable} if it is deterministic and, for any pair $\stateq, \stateq' \in \states$, there is at most one symbol $\sym \in \alphabet$ such that $\uwedge{\stateq}{\sym}{\stateq'} \in \trans$.
\end{definition}
% It is easy to see that $\log\nsymbols$-separability is a sufficient condition for compressing the representations of the symbols to the factor of $\log\nsymbols$.
% $\log\nsymbols$-separability is both necessary and sufficient for efficient compression with respect to the size of the alphabet.
% This is captured in the following lemma.
% \begin{lemma}
%     Let $\wfsa = \fsatuple$ be a deterministic FSA. 
%     Then, the exists an \hernnAcr{} simulating $\wfsa$'s transition function $\trans$ with the size $\bigO{\log\nsymbols \sqrt{\nstates}}$ if and only if $\wfsa$ is $\log\nsymbols$-separable.
% \end{lemma}
% \begin{proof}
% \end{proof}

$\log\nsymbols$-separability is a relatively restrictive condition.
To amend that, we introduce a simple procedure which, at the expense of enlarging the state space by a factor of $\nsymbols$, transforms a general deterministic (unweighted) FSA into a $\log\nsymbols$-separable one.
Since this procedure does not apply to weighted automata, it is presented in \cref{sec:log-separation}.\looseness=-1
